A Survey on Generative Modeling with Limited Data, Few Shots, and Zero Shot

Generative modeling in machine learning aims to synthesize new data samples that are statistically similar to those observed during training. While conventional generative models such as GANs and diffusion models typically assume access to large and diverse datasets, many real-world applications (e.g. in medicine, satellite imaging, and artistic domains) operate under limited data availability and strict constraints. In this survey, we examine Generative Modeling under Data Constraint (GM-DC), which includes limited-data, few-shot, and zero-shot settings. We present a unified perspective on the key challenges in GM-DC, including overfitting, frequency bias, and incompatible knowledge transfer, and discuss how these issues impact model performance. To systematically analyze this growing field, we introduce two novel taxonomies: one categorizing GM-DC tasks (e.g. unconditional vs. conditional generation, cross-domain adaptation, and subject-driven modeling), and another organizing methodological approaches (e.g. transfer learning, data augmentation, meta-learning, and frequency-aware modeling). Our study reviews over 230 papers, offering a comprehensive view across generative model types and constraint scenarios. We further analyze task-approach-method interactions using a Sankey diagram and highlight promising directions for future work, including adaptation of foundation models, holistic evaluation frameworks, and data-centric strategies for sample selection. This survey provides a timely and practical roadmap for researchers and practitioners aiming to advance generative modeling under limited data. Project website: https://sutd-visual-computing-group.github.io/gmdc-survey/.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/Extended_Review_Older_Version.tex <==

\section{Extended Review (Older Version)}

{\em In what follows, we give a brief description of the reviewed approaches so far (being updated gradually):}


%% TGAN - ECCV'18
\subsection{Transferring GAN (TGAN)}
Transferring GAN (TGAN) \cite{wang2018tgan} 
is the first systematic study to evaluate transfer learning in GANs. 
\cite{wang2018tgan} shows that using knowledge from GANs pre-trained on source domains with abundant data can shorten the convergence time and significantly improve the quality of the generated images in the target domain, particularly in cases where limited data is available from the target domain. 
The knowledge transfer is performed by using the pre-trained GAN for initializing the weights, and simply fine-tuning the weights on the data from the target domain using standard adversarial loss. 
TGAN evaluates various aspects of transferring a pre-trained GAN to a target domain including transfer configuration, size of the target dataset, the distance between source and target domains, and transferring knowledge to conditional GANs. 

\noindent
{\bf Transfer Configuration.} First, for evaluating the transfer learning configuration, they have considered four different configurations.
Considering two networks in a GAN (generator $G$, and discriminator $D$) each of them can be initialized either randomly (training from scratch) or with pre-trained weights (transfer learning by fine-tuning).
\cite{wang2018tgan} found that transferring the discriminator is more critical than transferring the generator, and improves results in both FID and IW metrics.
Transferring the generator only helps if the discriminator was already transferred; otherwise, it harms performance. 
Transferring both networks achieves the best result, and training is more stable in this setting, and this configuration is used for the rest of the experiments.
%In summary, networks adapted from pre-trained models generate high-quality images in significantly fewer iterations.

\noindent
{\bf Target Domain Size.}
TGAN \cite{wang2018tgan} compares transfer learning with training from scratch for different sizes of target datasets (1K, 5K, 10K, 50K, 100K, 500K, and 1M), and shows that transferring a pre-trained network always works better than training from scratch.
Specifically, improvement is more significant when the target data is more limited.
As an example, a GAN adapted from the pre-trained model requires roughly between two and five times fewer images to obtain a similar score than a GAN trained from scratch, meaning that adapting a pre-trained GAN can transfer relevant prior information for image generation in the target domain.

\noindent
{\bf Source and Target Domains.} 
One important contributing factor in transfer learning is the domain of the source model and its relation with the target model. 
To analyze this, \cite{wang2018tgan} evaluates different combinations of source and target domains for transfer learning. One interesting observation is that in some cases, in addition to the relation between source and target domains, the density of the source domain could be also very important for transfer learning in GANs. This is against the general practice for transfer learning in discriminative learning which always prefers knowledge transfer from a large and diverse dataset like ImageNet.
As an example, evaluation results in \cite{wang2018tgan} show that for the Flower \cite{nilsback2008automated} target domain, the pre-trained GAN on ImageNet is the best source model as it contains lots of flower classes. However, an interesting observation is that for the same target domain, using a pre-trained GAN on the semantically unrelated LSUN Bedrooms \cite{yu2015lsun} also results in competitive performance in terms of FID.


\noindent
{\bf Selecting Pre-trained GAN.}
\citet{wang2018tgan} believes that selecting a pre-trained model for GANs is more complicated compared to traditional transfer learning in discriminative tasks, as generation is a much more complex task than discrimination.
For this, \cite{wang2018tgan} proposes a metric to measure the correlation between source and target domains for image generation.
More specifically, the FID between generated samples by the pre-trained GAN $X_{gen}^{src}$, and the target data $X_{real}^{tgt}$ is shown to be a rough indicator of the correlation between source and target domains in the image generation.
However, \cite{wang2018tgan} mentions that in addition to this metric, the type of source data should also be considered as a GAN pre-trained in dense data seems to perform better than a GAN pre-trained on diverse data that have a large variation in image type.

\noindent
{\bf Transferring to cGAN.}
Finally, \cite{wang2018tgan} analyzes the efficacy of the transfer learning from an (unconditional) pre-trained GAN to a conditional GAN (cGAN).
For this study, they have used the ACGAN \cite{odena2017conditional, dumoulin2017a} as cGAN and compared training ACGAN from scratch and transferring a pre-trained GAN. Since in cGANs there are additional weights for conditioning on class/features, these conditional weights on classes are randomly initialized for transfer learning.
Results show that similar to unconditional GANs, transfer learning improves the convergence speed and the final performance of the ACGAN.

\noindent
{\color{magenta} \bf Remark.} TGAN has two major limitations: i) it uses WGAN-GP \cite{gulrajani2017improved} for the analysis which at the time of writing this survey is an outdated GAN, ii) it uses fine-tuning which is the most simple form of transfer learning and may result in distorting or forgetting a part of prior knowledge, especially when target data is limited.


%For a given target dataset, given a collection of pre-trained GANs, a way to estimate the most suitable model is desirable. However, choosing a pre-trained model suitable for GANs can be more challenging than in discriminative tasks. In generative scenarios, a much higher density of images per class is required to learn good transferable features for image generation than for image discrimination, where diversity seems more critical. For evaluating pre-trained GAN models, a good metric should measure the quality and diversity of the generated data. This work uses Fr\'echet Inception Distance (FID) and Independent Wasserstein (IW) as metrics to compare models. FID is the primary metric used since it is efficient to compute and correlates well with human perception. FID measures the similarity between two sets of datasets by calculating their Fr\'echet distance in an embedded space using an Inception model.
%The distance between the target data and the generated samples by the pre-trained model $(FID(X_{gen}^{src},X_{data}^{tgt}))$ is a helpful metric, as it takes the quality of the model into account.
%However, it has a rough correlation with the intended FID $(FID(X_{gen}^{tgt},X_{data}^{tgt}))$, which is the distance between generated target data and real target data. The latter is the desired FID as it evaluates the adapted GAN's performance in generating data from the target distribution. By comparing different configurations with FID, \citet{wang2018tgan} suggests that the density of the source dataset is more important than diversity and a dataset with one or few densely sampled classes is a better source model than more diverse datasets such as ImageNet or Places (even for apparently unrelated target domains). ImageNet and Places, while producing excellent transferable features for discrimination, seem not dense enough for generation, and LSUN data seems to be a better choice despite its limited diversity.






%% BSA - ICCV'19
\subsection{Batch Statistics Adaptation (BSA)} 
\citet{noguchi2019bsa} mention that when limited data is available from the target domain, fine-tuning the whole parameters of a pre-trained GAN (\eg 90 M trainable parameters), results in overfitting. To mitigate the issue, \cite{noguchi2019bsa} proposes to limit this update to a subset of parameters in GAN, more specifically, the scale and shift parameters of the batch normalization (BN) in each layer of the $G$.
First, they discuss the scale and shift parameters from the lens of filter selection. Applying the scale and shift parameters to the output of the convolutional layer can be considered as follows:
\begin{equation}
\label{eqn:bsa_scaleshift}
\begin{aligned}
& conv(x;W).\gamma + \beta \\
& = conv(x;W.\gamma + \beta) \\
& = conv(x;\{ \gamma_1 W_1 + \beta_1 , ... , \gamma_N W_N + \beta_N \} )
\end{aligned}
\end{equation}
where $W_i$ denotes the $i^{th}$ filter in a convolutional layer.
\cite{noguchi2019bsa} mentions that considering Eqn. \ref{eqn:bsa_scaleshift}, the scale $\gamma$ controls the strength of a filter and $\beta$ controls the activation threshold.
For example, where $\gamma_i$ and $\beta_i$ are large, the corresponding filter becomes easy to activate. Therefore these parameters are controlling the activation of the filters.
Then, to understand the effect of the BN parameters on encoding class-related information, an analysis was performed on the SNGAN projection \cite{miyato2018spectral, miyato2018cgans} which is a conditional GAN that uses different batch normalization parameters for each class.
The T-SNE plots of these parameters show that similar BN parameters are used for semantically similar classes.
Based on this observation, they propose to freeze all the weights of the $G$ to the pre-trained weights and only update the scale and shift parameters of the BN layer.

\noindent
In addition, they propose a supervised learning approach instead of adversarial learning of the GAN during the adaptation.
For this, both latent code and the BN parameters of the $G$ are updated during training to enable supervised learning.
Specifically, inspired by Generative Latent Optimization \cite{bojanowski2018optimizing}, latent code is optimized to find the corresponding latent vector $z_i$ for each real sample $x_i$, and BN parameters are updated to adapt the generator to the new domain.
This is achieved by minimizing the distance between $G(z_i)$ and $x_i$ using both an $L_1$ loss in the image space, and the perceptual loss \cite{johnson2016perceptual} in the feature space of a pre-trained classifier $C$ (VGG16 \cite{simonyan2014very}). Two additional terms are used to regularize both $z$ and BN parameters during training.

%\begin{equation}
%\label{eq:bsa_loss}
%\begin{aligned}
%\mathcal{L}_{BSA} = 
%& \mathbb{E}_{i} \{ \|x_i - G(z_i + \epsilon) \| \} \\
%& \mathbb{E}_{i} \mathbb{E}_{l} \{ \|C^l(x_i) - C^l(G(z_i + \epsilon)) \| \} \\
%& + ...
%\end{aligned}
%\end{equation}

\noindent
{\color{magenta} \bf Remark.}
BSA has two major limitations: i) updating only BN parameters limits the adaptation capability of the BSA, ii) using the $L_1$ loss on pixel space results in blurry image generation.

% MineGAN - CVPR'20
\subsection{MineGAN}
The process of mining GANs is introduced in \cite{wang2020minegan}, where a miner network is learned to sample from a region of the code distribution $p(z)$ of the pre-trained GAN that is most close to the target samples. 
More specifically, an MLP network $M$ is learned to minimize the adversarial loss during adapting a pre-trained GAN to a target domain with limited data:
\begin{equation}
\begin{aligned}
    & \mathcal{L}^{M}_{D} = 
    \mathbb{E}_{z \sim p(z)} [ D(G(M(z))) ] - \mathbb{E}_{x \sim p(x)} [ D(x) ] \\
    & \mathcal{L}^{M}_{G} = -
    \mathbb{E}_{z \sim p(z)} [ D(G(M(z))) ]
\end{aligned}
\end{equation}
The learning algorithm has two main steps. First, the mining GAN is trained using the samples from the target data. In this step, starting from a pre-trained GAN, $M$ is trained from scratch, $G$ is frozen, and $D$ is fine-tuned.
After training $M$, all three networks are fine-tuned in the second step.

\noindent
The idea of mining GAN is also extended to two other scenarios: i) mining multiple GANs, and ii) conditional MineGAN.
For mining from multiple pre-trained GANs, a separate miner network $M_i$ is used for each of the GANs $G_i$. 
In addition, a selector module is appended that tracks the number of successful generations from each GAN (based on the discriminator's output), and based on this, a multinomial distribution is assigned over GANs to select the GAN for image generation during inference. 
To extend the idea to conditional image generation, two separate miners are used to output the latent code and the conditions on feature maps.

\noindent {\color{magenta} \bf Remark. }
The major limitation of the MineGAN is that it searches the latent space of the GAN to find the related prior knowledge instead of the weights of the network. Note that this is challenging because the encoded knowledge in the latent space is even harder to interpret compared to the weights of a GAN \cite{harkonen2020ganspace}.
However, combining this algorithm with knowledge-preserving approaches may improve performance.
For this, MineGAN++ \cite{wang2021minegan++} adds the discriminator regularization to MineGAN by only updating the sensitive parameters to the target domain and freezing the least important ones.
%Note that a different approach is shown to be more efficient in EWC \cite{li2020ewc}, where the change on important layers are penalized more.


% FreezD - CVPR'20 workshop
\subsection{Freeze the Discriminator (FreezeD)}
In discriminative learning, it is well-known that the earlier layers of the CNNs encode the general knowledge and the later layers encode task-specific knowledge \cite{yosinski2014transferable}.
Since the discriminator performs a discriminative task during training GAN, \cite{mo2020freezed} mentions that early layers of the $D$ similarly encode the general knowledge and could be similar for source and target domains when transferring a GAN.
Therefore, to prevent overfitting during adapting a GAN under limited data and preserve the general encoded knowledge in $D$, they propose to freeze the early layers of $D$ and fine-tune all other layers of GAN (including all layers of $G$) during adapting to the target domain. 
This simple baseline is shown to be very effective for transferring both unconditional and conditional GANs.

% AdaFM - ICML'20
\subsection{Leveraging Pretrained GANs with Adaptive Filter Modulation (AdaFM)}
In order to efficiently leverage a pre-trained GAN for image generation on a target domain with limited data, \citet{zhao2020leveraging} aims to reuse the general knowledge of the pre-trained GAN and update the domain-specific part.
With this aim, first, they identify the general and domain-specific parts of a GP-GAN by freezing and fine-tuning various combinations of the layers in both $G$ and $D$.
The experimental results show that lower-level kernels (the ones closer to the observation $x$ in both $G$ and $D$) encode general knowledge and the higher-level kernels (closer to the decision in $D$, and closer to input noise $z$ in $G$) encode the domain-specific knowledge.
The domain-specific knowledge is supposed to be updated during adaptation and the general knowledge is supposed to be preserved.
As the domain-specific part could include a large number of the trainable parameters, a smaller structure is proposed which includes one FC layer, and two style blocks inspired by StyleGAN \cite{karras2019style}.
To preserve the knowledge of the general part (kernels in low-level layers), the pre-trained kernels within these layers are frozen. In addition, to add more flexibility, an adaptive filter modulation (AdaFM) is proposed. 
Specifically, for the weights of a convolutional layer $\mathbf{W} \in \mathbb{R}^{C_{out} \times C_{in} \times k \times k}$, a scale and shift parameter is trained for each $k \times k$ kernel to modulate the weights for new domain:
\begin{equation}
    \mathbf{W}^{AdaFM}_{i,j,:,:} = 
 \mathbf{\gamma_{i,j}} \mathbf{W}_{i,j,:,:} + \mathbf{\beta_{i,j}}
\end{equation}
Note that the pre-trained kernels are frozen during adaptation and only the scale and shift parameters of the modulation operator are learned.

% EWC - NeurIPS'20
\subsection{Elastic Weight Consolidation (EWC)}
\citet{li2020ewc} explore the concept of few-shot image generation (FSIG), which aims to train a GAN to generate diverse and high-quality images using only a few samples, \eg only 10-shots.
It is unreasonable to expect a GAN to learn the whole data distribution using only 10 samples. Therefore, a GAN pre-trained on a related source domain is leveraged.
Then, the FSIG task can be considered as preserving the diversity of the source domain while adapting to the style of the target domain.
This challenging task is addressed in \cite{li2020ewc} by considering the key property that different weights in deep neural networks have no equal importance for handling a task. 
For this, \cite{li2020ewc} aims to address two main questions: i) which weights are more important to preserve, and which weights have more freedom to be updated? ii) How to quantify the importance and regularize it by a loss function?

\noindent
To answer these questions, first, an analysis is performed to investigate the rate of change when adapting a DCGAN pre-trained on CelebA to emoji’s dataset with abundant data. Their analysis shows that the rate of change is different for various layers. The layers with less change seem to have more general knowledge (shared between two domains), and therefore they are more important to preserve.
Then, inspired by Elastic Weight Consolidation (EWC) \cite{kirkpatrick2017ewcmethod} --which is proposed to measure and preserve the important weights for a task in continual learning of discriminative tasks-- \cite{li2020ewc} uses the Fisher information $F$ to measure the importance of the weights:
\begin{equation}
\label{eqn:Fisher_EWC}
F = \mathbb{E}[-\frac{\partial^2}{\partial\theta_S^2}L(X|\theta_S)]
\end{equation}
where $\theta_S$ denotes the weights of the GAN pre-trained on the source domain, $X$ is a set of generated images with pre-trained GAN, and $L(X|\theta_S)$ denotes the loss computed by the discriminator. 
Note that $F$ has the same dimension as $\theta_S$ meaning that for each parameter of the network $\theta_{S,i}$, there is a related importance value $F_i$.
Then the fisher information values are used to define a regularizer to penalize the change in the parameters of the source network based on their importance for image generation in the source domain.
This regularizer is added to the standard adversarial loss when adapting to the new domain:
\begin{equation}
\label{eqn:Loss_EWC}
\mathcal{L}_{EWC} = \mathcal{L}_{adv} + \lambda \sum_i F_i (\theta_i - \theta_{S,i})^2
\end{equation}
where $\lambda$ is the regularization weight.
One major benefit of this loss function / approach is that no new parameters are introduced meaning that no tedious manual design on new parameters is required.

\noindent
{\color{magenta} \bf Remark.}
The FI metric used in EWC \cite{li2020ewc} is a simple and powerful metric to measure and preserve the important weights / encoded knowledge during adaptation, but as this importance is measured on the source domain, it assumes that the parameters have the same importance for both source and target domains.
Even though this assumption could be reasonable for very close source-target domains (Adult Faces $\rightarrow$ Baby Faces), it may not stay valid for a target domain that is far from the source domain (Human Faces $\rightarrow$ Cat Faces).

%As it is unreasonable to expect to fully infer the data distribution from just a few observations, we seek to leverage a large, related source domain as pre-training. Thus, we wish to preserve the diversity of the source domain, while adapting to the appearance of the target.


%\citet{li2020few} consider the problem of few-shot image generation as a continuous learning framework as it is naturally a process of sequentially learning two tasks. Also, the underlying assumption is that the source and target domains share some latent factors, with some differences related to their distinct difference in appearance. For example, when transferring from real natural faces to emojis, variations in pose and expression can be naturally extended to the target domain. Since in the FSIG scheme, there are only a few training examples, it is necessary to distill knowledge learned from the previous source domain and try not to forget the diversity in the source domain in order to combine it with the style from the limited data of the target domain to generate more diverse results. However, after the adaptation, it is no more possible to generate the data in the source domain and there will always be an inherent trade-off between preserving information from the source and adapting to the target domain.
%\citet{kirkpatrick2017ewcmethod} have proposed Elastic Weight Consolidation (EWC), which evaluates the importance of each parameter, in a discriminative modeling setting, by estimating its Fisher Information relative to the objective likelihood. \citet{li2020few} apply the EWC technique in a generative setting (FSIG) and regularize the changes of the weights during this adaptation. They propose to quantify the “importance” of model weights, emphasizing the preservation of important parameters during the tuning process.

%\citet{li2020few} first assume there is abundant data in the target domain to learn a decent generative model and expect to get some inspiration on what good weights look like. They analyze the rate of change of the generator weights between the source and the target-adapted model (as it is important to know which weights change significantly when switching to learning another distribution) and observe that the weights in the last layer of the network change the least on average compared to other early layers. This implies that when adapting with a few examples, some weights in the last layer are more important and should be better preserved than those in other layers. To quantify the importance of each weight, the Fisher information F is calculated. Given a pretrained generative model on the source domain, by generating a certain amount of data X, given the learned values of network parameters $\theta_S$, the Fisher information F can be computed as:

%As the weights in the last layer have much higher F than those in other layers and given the observation that the weights in the last layer of the network change the least on average compared to other early layers, they directly use F as an ‘’importance measure’’ for weights and add a regularization loss to penalize the weight change during the adaptation to the target domain. Therefore, the weights in different layers will be regularized differently during the adaptation to the target domain as follows:

%where $\theta_S$ represents the weights learned from the source domain, $i$ is the index of each parameter of the model, and $\lambda$ is the regularization weight to balance different losses. The second term in Equation \ref{eqn:Loss_EWC} was first proposed in \citet{kirkpatrick2017ewcmethod} for the classification task and called the Elastic Weight Consolidation (EWC) loss and \citet{li2020few} uses this term to demonstrate its effectiveness in the few-shot generative setting. Since the number of parameters is significantly larger than the number of examples, without this regularization to preserve the diversity from the source ($\lambda$=0), the model adaptation with a few examples in the target domain will quickly result in over-fitting, which manifests as re-generating almost replicas of only the given target examples.

%They evaluate the proposed method against three others: \textbf{NST} (\citet{gatys2016image}), \textbf{BSA} (\citet{noguchi2019image}), and \textbf{Mine-GAN} (\citet{}). The Neural Style (NST) work of [6] represents a family of neural style transfer methods as an adaptation to a new domain can be also regarded as a style transfer task. As it is an example-based method, we randomly select one image from the small number of target examples to stylize an image sampled from the source data. Both BSA and Mine-GAN also focus on adapting models from a source to a target domain but they introduce additional parameters. The BSA method  is adding new batch norm layers into the original BigGAN generator and learns new parameters only during the adaptation. The MineGAN approach adds a small mining network M in front of the original Progressive GAN generator and proposes a two-stage fine-tuning strategy (i.e., fine-tune M first and then fine-tune M jointly with the generator). For all experiments, they use the StyleGAN \citet{karras2019style} framework.



% SVD - arxiv'21
\subsection{Few-shot Adaptation of Generative Adversarial Networks}
\citet{robb2020svd} aims to find a more efficient and constrained parameter space to prevent overfitting while adapting a GAN to a target domain. For this, they apply singular value decomposition (SVD) \cite{van1976generalizing} separately on each layer of both $G$ and $D$: $W^{(\ell)} = (U \Sigma V^T)^{(\ell)}$, where $U$ and $V$ are singular vectors, and $\Sigma$ denotes singular values.
Then, \cite{robb2020svd} shows that varying the singular values is related to changing entanglement between different attributes within data, and therefore it just updated the singular values of all layers when adapting to a new domain.


% GAN Memory - NeurIPS'20
\subsection{GAN Memory with no Forgetting / CAM GAN}
GAN memory with no forgetting \cite{cong2020ganmemory} aims to address continual learning setup in generative learning, \ie, a GAN that continually learns to generate images from different domains without forgetting the knowledge of image generation for previous domains.
First, they perform an experiment to show that by modulating the weights (FC and Conv layers) of a GAN well-trained on the source domain (without changing the source parameters), the modulated GAN can be trained to generate high-quality and diverse images from a perceptually-distant target domain.
For this experiment, they use the modified version of the AdaFM \cite{zhao2020leveraging} by normalizing the weights before applying the modulation.
Then, this modulation is used to achieve continual generative learning, by starting from a well-trained GAN as the base, freezing the weights of this GAN, and only learning the modulation parameters for the new domain.
The modulation parameters are then proposed to be compressed using a progressive approach \cite{schwarz2018progress} that learns a shared set for all of the modulation weights using matrix factorization and low-rank regularization.
CAM GAN \cite{varshney2021camgan} extends the idea by applying a more parameter-efficient transformation instead of the AdaFM modulation used in GAN Memory.




% GenDA - arxiv'21
\subsection{One-shot Generative Domain Adaptation (GenDA)}
One-shot Generative Domain Adaptation (GenDA) \cite{yang2021genda} addresses the challenging problem of transferring  a pre-trained GAN on a source domain to a target domain using only one image from the target domain ---one-shot image generation.
To prevent collapsing GAN to one image during adaptation and preserve the diversity of the source domain, \citet{yang2021genda} freeze the whole parameters in the generator and discriminator and proposes three different modules during adaptation.
First, inspired by the fact that some knowledge is encoded in the latent space of the GAN, a lightweight attribute adaptor is applied on input $z$ in the form of a scale and shift operation to adapt the latent space to the target domain.
Second, they propose an attribute classifier by discarding the pre-trained head of the $D$ and adding a lightweight attribute classifier.
Finally, a truncation trick is applied to the transformed latent space to preserve the diversity of the source domain during adaptation.



% CDC - CVPR'21
\subsection{Cross-Domain Consistency (CDC)}
Transfer learning \cite{wang2018tgan} and data augmentation \cite{karras2020ada} are two successful approaches that are introduced to address training GANs under limited data.
However, most of these approaches are designed for scenarios with more than 100 images from the target domain.
When only 10 images from the target domain are available, GAN severely overfits these samples, \ie during training / adapting GAN, the discriminator $D$ easily memorizes these samples and enforces the $G$ to generate the same samples to minimize the loss value on the fake samples.

\noindent
One observation about this overfitting, is discussed in \cite{ojha2021cdc}. Consider a pre-trained GAN that can generate high-quality and diverse images from the source domain. By tracking a set of noise vectors ($\{ z_i \}$), \cite{ojha2021cdc} mentions that all these diverse samples ($\{ G_s(z_i) \}$) collapse to a set of similar samples ($\{ G_t(z_i) \}$) after simple fine-tuning \cite{wang2018tgan} on target samples.
Therefore the similarities and differences between these samples are removed after fine-tuning.
To keep the diversity of the generated samples by $G_s$ on $G_t$, a cross-domain correspondence (CDC) loss is proposed in \cite{ojha2021cdc}.
Specifically, during each iteration of adapting $G_s$ to $G_t$, a set of $N+1$ noise vectors $\{ z_0, ..., z_N \}$ are sampled.
Then, for each sample, the pair-wise similarities with all remaining samples in the feature space are computed on all layers of the generator and converted to probabilities using Softmax. This process is performed before and after adapting the GAN resulting in the following probability vectors:
\begin{equation}
\label{eqn:cdc_probablity}
    \begin{aligned}
     & y_i^{s,l} = Softmax[\{sim(G_s^l(z_i),G_s^l(z_j))\}_{\forall i \neq j}]  \\
     & y_i^{t,l} = Softmax[\{sim(G_t^l(z_i),G_t^l(z_j))\}_{\forall i \neq j}]
    \end{aligned}
\end{equation}
Then, the KL-divergence between these two vectors (for all layers of $G$ and all noise samples) is added as a diversity-preserving regularizer to the standard adversarial loss during adapting GAN to the target domain:
\begin{equation}
\label{eqn:cdc_loss}
    \mathcal{L}_{CDC}= \mathbb{E}_{z_i} \Sigma_{l,i} D_{KL} (y_i^{t,l} \| y_i^{s,l})
\end{equation}
In addition, as few samples only represent a small subset of the target distribution, \cite{ojha2021cdc} extends this notion to the latent space of the GAN by defining an anchor region $\mathcal{Z}_{anch}$ as a subset of the whole latent space.
When the random noise is sampled from this anchor region, the corresponding generated image is processed with the image level discriminator $D_{img}$, otherwise, it is passed to a patch-level discriminator $D_{patch}$.

\noindent
{\color{magenta} \bf Remark.}
CDC has two major limitations: keeping the corresponding similarity between source and target domains is only applicable to similar domains (\eg Human Face $\rightarrow$ Face Sketches) where there is a one-to-one correspondence between them and it can not generalize to distant domains (\eg Human Face $\rightarrow$ Cars), ii) the diversity preservation is only applied to $G$ without applying any mechanism to preserve the knowledge in $D$.


% KD for FSIG - ICLR'22 withdrawn
\subsection{Exploiting Knowledge Distillation for Few-Shot Image Generation}
To preserve the diversity within $G_s$ while adapting to the new domain, \citet{hou2022exploitingkd} exploit knowledge distillation idea by treating source model as teacher and the target model as student.
A momentum relation distillation is introduced for the generator that uses the SSIM of the feature maps as relation between samples in the source and target domains, and aims to preserve this relation using the query-key formulation. O extend the key list, inspired by momentum contrastive learning \cite{he2020momentum}, a generator with momentum update is used to generate the keys for target domain.


\subsection{C3: Contrastive Learning for Cross-domain Correspondence in Few-shot Image Generation}
Contrastive Learning for Cross-domain Correspondence ($C^3$) ~\cite{Lee2021C3} proposes to use contrastive learning to prevent overfitting the target GAN to the real samples.
Contrastive learning is defined by considering the generated image by source GAN for a specific latent code $G_s(z_i)$ as an anchor point. Then, the generated images for the same latent code with the. adapted generator ($G_t(z_i)$) is considered as positive pair, and the generated samples with the adapted generator for other latent code values ($G_t(z_j)$, $i \neq j$) are considered as negative pairs. 


% DCL - CVPR'22
\subsection{Dual Contrastive Learning (DCL)}
\citet{zhao2022dcl} propose a framework for separate analysis of the quality and diversity of the generated images during adapting a pre-trained GAN to a target domain with few samples (10-shot) using different approaches.
For analyzing the quality of a generated image, a classifier is used as a proxy. More specifically, the binary classifier $C$ is trained on the source and target images and then is applied to the generated images. The soft output $p_t$ of this classifier predicts the probability of belonging to the target domain. Finally, the average value of $p_t$ over 1000 generated images is used as a quality indicator.
The intra-LPIPS metric \cite{ojha2021cdc} for generated images is used to measure the diversity.
The results of this analysis suggest that all FSIG approaches achieve similar generation quality and the methods that can slow down the diversity degradation during adaptation can finally achieve higher image generation performance.

\noindent
Based on this observation, they propose a method to preserve the diversity of the source GAN during adaption to the target domain.
More specifically, they propose to maximize the mutual information between the features of the generated images before and after adaptation for all layers of the network:
\begin{equation}
\label{eqn:dcl_mi}
    \argmax MI \{ \pi^l(G_t(z_i)), \pi^l(G_s(z_i)) \}
\end{equation}
where $\pi^l$ is an embedding function to extract the $l^{th}$ level features.
Since it is challenging to directly maximize the MI \cite{paninski2003estimation}, contrastive learning \cite{oord2018representation, henaff2020data} is applied to solve Eqn. \ref{eqn:dcl_mi}.
More specifically, the dual contrastive loss (DCL) is proposed which considers diversity preservation for both $G$ and $D$.
For $G$, the generated images by the source and adapted GAN with the same $z$ are used as positive pairs, and the generated image for other $z$ values (one source and one target) are used as negative pairs.
For $D$, the agreement between discriminative features of generated images with the same $z$ in source and adapted GANs (by $D(G_s(z_i))$, and $D(G_t(z_i))$) is increased by considering them as positive pair, and the training is regularized by pushing away the discriminative features of the real images from them as a negative pair.


% RSSA - CVPR'22
\subsection{Relaxed Structural Similarity Alignment (RSSA)}
\citet{xiao2022rssa} extends the cross-domain consistency idea of the CDC \cite{ojha2021cdc} to a more constrained form termed relaxed spatial structural similarity (RSSA).
RSSA uses two separate regularizers to maintain the diversity of the pre-trained GAN with constraining the structural similarity.
First, a self-correlation consistency loss is introduced to maintain the inner correlation of the feature maps for the same random noise before and after adaptation.
More specifically, considering the feature maps $f^l \in \mathbb{R}^{c \times w \times h}$ at $l^{th}$ layer of the $G$ for a random noise $z_i$, $f^l(x,y)$ is a $c$ dimensional vector presenting a spatial location.
Then, the correlation between this location and all other locations of the feature map is calculated using the cosine similarity as follows:
\begin{equation}
\label{eqn:rssa_similarity}
    C^l_{x,y}(i,j) = cos(f^l(x,y), f^l(i,j))
\end{equation}
resulting in a self-correlation matrix $C^l_{x,y} \in \mathbb{R}^{w \times h}$ for each spatial location.
Then, the self-correlation is enforced to stay the same before and after adapting the GAN to a target domain for all layers of the GAN:
\begin{equation}
\label{eqn:rssa_selfcorrelation_loss}
    \mathcal{L}_{RSSA}^{scc} = \sum_l \sum_{x,y} {smooth}_{L_1} (C^{s,l}_{x,y} , C^{t,l}_{x,y})
\end{equation}
Then, considering the continuous nature of the latent space in GANs, for a random noise $z_i$ a neighborhood is defined, and the spatial structural similarity between the images generated by $z_i$ and generated by the noise sampled from this area is measured in a similar manner and enforced to be same for the pre-trained and the adapted GAN.
Finally, RSSA introduces a latent space compression with the aim of finding the most proper subspace in the latent space for generating samples for the target domain.
This space is determined by inverting the target samples into the extended latent space $\mathcal{W^+}$ of the StyleGAN using Image2StyleGAN \cite{abdal2019image2stylegan} inversion approach and projection of these inverted samples into $z$ space. This is a similar concept to the latent optimization introduced for the $L_1$ loss in BSA \cite{noguchi2019bsa}.

\noindent
In addition, RSSA introduces a new metric as generation quality in the few-shot setup that considers the structural consistency between the samples generated by the source and adapted GANs.
Structural consistency score (SCS) between a pair of images --generated by the source GAN and adapted GAN using the same noise input-- is obtained by first extracting the edge map \cite{xie2015holistically} for each of the images, and then computing the dice similarity coefficient \cite{dice1945measures} between these feature maps.
The average value over a set of samples is considered as the SCS between two GANs.

\noindent
{\color{magenta} \bf Remark.}
RSSA poses too much constraint on the structural similarity (similar to one-shot approaches) that limits the adaptation capability, especially for the target domains which might not be a one-to-one relation between semantics.
Similar to CDC, the importance of knowledge preservation for the discriminator is not considered.






% JoJoGAN - ECCV'22
\subsection{JoJoGAN}
JoJoGAN \cite{chong2022jojogan} addresses one-shot image generation using the style space of the StyleGAN.
More specifically, the first GAN inversion is used to find the corresponding style code in the extended latent space of the StyleGAN.
Then, using the inverted style code, the style mixing is used to generate a set of styles $\{ s_i \}$ related to the reference image.
These styles are supposed to be close to the target image.
Then, the parameters of the source GAN are updated in a way to minimize the perceptual loss between the target image and generated image by each of these style codes in the style set.
Then, the adapted GAN can be used to generate images from the target domain.

% MDL - ECCV'22
\subsection{Few-Shot Image Generation with Mixup-based Distance Learning (MDL)}
\citet{kong2022mdl} aims to address pretraining-free few-shot image generation. 
\cite{kong2022mdl} mentions that overfitting a GAN under limited data can be observed by discontinuous latent interpolation (stairlike latent space) and overly confident discriminator.
To prevent this, MDL aims to  preserve the modes and learn interpolable latent space.
First, an anchor point in the latent space is defined by the weighted average of $N$ random latent codes: $z_0 = \sum_{i=1}^N c_i z_i$, where weights are drawn from a Dirichlet distribution $\mathbf{c}=[c_1, ..., c_N]^T$, $\mathbf{c} \sim Dir(\alpha_1, ..., \alpha_N)$.
Then, similar to CDC \cite{ojha2021cdc}, the pairwise similarity between the generated image with anchor point $z_0$, and all generated images with other latent codes are computed as an N-way probability distribution $p_G$.
Then, softmax is applied to the components of $\mathbf{c}$ to produce the distribution over latent codes $p_z$.
The KL-divergence between $p_G$ and $p_z$ is added to prevent mode collapse in $G$.
For $D$, the projected feature maps from the penultimate layer of $D$ are used to compute a distribution over features $p_D$ for generated images with the same latent codes.
Finally, the KL-divergence between $p_D$ and $p_z$ is added to adversarial loss to prevent overfitting $D$ to real samples.


% CtlGAN - arXiv'22
\subsection{Contrastive Transfer Learning (CtL) for Few-Shot Portraits Generation}
\citet{wang2022ctlgan} addresses the portrait generation from the real images using the few-shot image generation instead of using the traditional framework of image-to-image translation.
Given a real image, an encoder is used to encode it into a latent code.
Then the decoder generates stylized images from that latent code.
The decoder is a generator $G$ of a pre-trained StyleGAN2 that is adapted to the target domain using a few samples.
To preserve the diversity, during adaptation a contrastive loss is proposed. For each latent code $z_i$, the generated image from the same latent code using source and adapted $G$ are considered positive pair, and the generated images using other latent codes with adapted $G$ are considered as negative pairs.
In addition, similar to CDC, an additional consistency loss is proposed that aims to preserve the similarities in the distribution of input features to Adaptive Instance Normalization (AdaIN) blocks of StyleGAN2, before and after adapting the generator to the target domain.

\noindent
{\color{magenta} \bf Remark.} Contrastive learning; GAN inversion; cross-domain similarity.

% AdAM - NeurIPS'22
\subsection{Adaptation-Aware kernel Modulation (AdAM)}
Adaptation-Aware kernel Modulation (AdAM) \cite{zhao2022adam} mentions that one major limitation of the FSIG approaches is that they only consider the source domain for preserving the knowledge. For example, EWC \cite{li2020ewc} penalizes the change in the weights that are important for image generation in the source domain, or CDC \cite{ojha2021cdc} aims to preserve the diversity of the source GAN by transferring the pair-wise similarity / difference to the target domain.
AdAM mentions that considering the target domain for knowledge preservation can mitigate this problem and enable the model adaptation to distant domains ---called general FSIG in \cite{zhao2022adam}.

\noindent
There are two major contributions in \cite{zhao2022adam}. First, it is mentioned that all previous works just focus on the close domains for FSIG, \eg Human Faces $\rightarrow$ Human Face Sketches. Once this assumption is relaxed (\eg Human Faces $\rightarrow$ Car Faces), all these approaches perform no better than simple fine-tuning in TGAN \cite{wang2018tgan}, and \cite{zhao2022adam}  believes that this happens because these algorithms do not consider the target domain when designing knowledge preservation approaches.
The second contribution aims to address this problem with an adaptation-aware FSIG approach which includes two main modules.
First, a low-light importance probing mechanism is used to evaluate the importance of each kernel of $G$ and $D$ when adapting from source to target domain. This results in a set of important kernels that should be preserved during adaptation, and a set of unimportant kernels that can be updated to let the GAN adapt to the target domain with more flexibility.
The important kernels are preserved by applying the low-rank kernel modulation \cite{milad2021revisit} approach which learns some residual modulation weights for a controlled adaptation to the target domain.
The remaining kernels are simply fine-tuned.
Results show that AdAM performs significantly better than previous approaches on general FSIG (both close and distant domains).

\subsection{Fair Generative Models via Transfer Learning (FairTL)}
Fair Generative Models via Transfer Learning (FairTL) \cite{teo2023fairtl} adopts transfer learning in GANs to train a fair generative model \wrt a sensitive attribute (SA) using a limited fair dataset.
Specifically, fairness is defined as equal representation in GANs. For example, a generative model that generates male and female images with the same probability is considered to be fair \wrt SA Gender.
FairTL shows that by simply fine-tuning a (potentially biased) pre-trained GAN on a small fair dataset, the fairness of image generation can be improved.
Then two additional modules are proposed to prevent the mode collapse on this limited data.
First, a frozen discriminator is added to evolving discriminator during adaptation to a fair dataset to preserve the quality of the generated images.
Then, a linear probing stage is applied before fine-tuning the earlier layers to preserve the general knowledge during adaptation to the target fair dataset.

\subsection{Few-Shot Image Generation via Latent Code Learning (LCL)}
\citet{mondal2023lcl} proposes a latent code learner that learns to map the input latent code (Gaussian noise) to the extended intermediate latent code space of a StyleGAN2 to enable sample generation from a different domain without fine-tuning the generator $G$ pre-trained on a source domain.
To train this latent code learner, a style matching loss and an adversarial loss are proposed.
More specifically, the style matching loss compares the generated image and the target image in the embedding space of a pre-trained VGG19 model \cite{simonyan2014very} to make sure generated samples follow the style of the target samples.
In addition, similar to standard adversarial training, the discriminator is fine-tuned and aims to discriminate between real and fake samples.
The latent code learner is then optimized to minimize both adversarial loss and style-matching loss.
For generating each new batch of images from a target domain, a new latent coder is trained from scratch.
This has been shown to increase the diversity of generated samples, however, it increases the computational complexity of sample generation.


\subsection{Removing InCompatible Knowledge (RICK)}
The impact of incompatible knowledge transfer in FSIG is discovered in \cite{zhao2023rick}, and it is shown that Removing InCompatible Knowledge (RICK) could be beneficial when adapting to a target domain.
RICK proposes two major contributions for FSIG.
First, by applying the GAN dissection \cite{bau2018gandissection, bau2017networkdissection} with importance probing during adaptation \cite{zhao2022adam}, \cite{zhao2023rick} shows the incompatible knowledge transfer roots from the least important kernels during adaptation (measured by Fisher information).
One interesting observation is that this incompatible knowledge is not being removed by simple fine-tuning.
Then, based on this analysis, they propose to prune the incompatible filters during adapting the pre-trained GAN to the target domain.
More specifically, during adapting the pre-trained GAN to the target domain, after each $N$ iteration, the importance of the filters during this adaptation is measured using FI, similar to \cite{zhao2022adam}. However, note that in contrast to \cite{zhao2022adam}, RICK uses dynamic importance probing integrated into the main adaptation phase, rather than being a separate phase.
After measuring the importance of the kernels during adaptation, all kernels are classified into three groups based on their importance: i) the least important kernels are pruned (removed from the adaptation process permanently) to stop incompatible knowledge transfer to the target domain, ii) the important kernels are frozen to preserve their knowledge, and iii) remaining kernels are fine-tuned to enable the model to capture target domain knowledge.



% Visual Prompt Tuning (Google) - CVPR'23
\subsection{Visual Prompt Tuning for Generative Transfer Learning}
{\bf Background.}
Even though GANs can generate high-fidelity images, likelihood-based models like VAEs have the benefit of more diverse image generation due to better distribution coverage \cite{vahdat2020nvae, van2016conditional}.
Due to the challenges of direct maximization of the likelihood in pixel space, Vector-Qunatized VAE (VQ-VAE) 
\cite{razavi2019generating, van2017neural} proposes a two-stage process for image generation.
In the first stage, known as {\bf tokenization}, the image is compressed into discrete latent space (visual tokens) using three major components: i) an encoder $E$ that maps images $x$ into an embedding space E(x), ii) a codebook $\mathbf{e}_k$, $k \in 1, \dots, K$ that quantizes the embeddings into visual tokens (indices), acting like a lookup table, and iii) a decoder $G$ that learns to reconstruct the image $\hat{x}$ from visual tokens $\mathbf{e}$.
In the second stage, a latent prior of the visual tokens is predicted (usually using a transformer), and then the decoder from the first stage is used to map the tokens into the image space.
From the perspective of predicting the latent prior of visual tokens, these works can be broadly categorized into two types. AutoRegressive (AR) approaches like DALL$\cdot$E \cite{ramesh2021dalle} and VQ-GAN \cite{esser2021vqgan}, learn an AR predictor that follows a raster scan order that predicts the visual tokens from left to right, line-by-line. 
Non-AutoRegressive (NAR) approaches like DALL$\cdot$E2 \cite{ramesh2022dalle2}, MaskGIT \cite{chang2022maskgit}, Latent Diffusion \cite{rombach2022latentdiffusion}, or Imagen \cite{saharia2022imagen} usually resort to masking techniques \cite{devlin2019bert} to learn to predict the visual tokens in a series of refinement or denoising steps.
Starting from a blank canvas where all visual tokens are masked, NAR approaches unmask a set of tokens (in random places) in each step, and the remaining ones are unmasked in the next iterations.

\noindent
Visual Prompt Tuning \cite{sohn2023vpt} is the first work that adopts the prompt tuning idea for image generation with generative knowledge transfer.
\citet{sohn2023vpt} base their framework on VQ-VAE where a pre-trained MaskGIT\cite{chang2022maskgit} / VQ-GAN\cite{esser2021vqgan} on the ImageNet dataset, as an example of NAR /AR approach  is used as initialization.
Then, during adaptation, all the parameters of the VQ Encoder, VQ decoder, and transformer are frozen, and a generator is learned to minimize the adaptation loss by generating and appending a set of visual tokens to the predicted prior.
These visual tokens guide the generation process for the target domain by helping the transformer to predict proper tokens to the VQ decoder.
The visual token generator takes conditional variables (\eg, class, instance, position, and factor) to generate the visual tokens, and efficient design is designed through factorization of the MLP networks to prevent parameter overhead.
Additionally, a new prompt design named "Marquee Header" is proposed which increases the diversity by interpolating between instance and class conditions, or interpolating between two instances.


\subsection{Instance-Conditioned GAN (IC-GAN)}
To model complex distributions like ImageNet, Instance-Conditional GAN (IC-GAN) \cite{casanova2021icgan} assumes some clusters in the features space of the training data and aims to learn data distribution conditioned on these clusters, \ie, as a mixture of conditional distributions.
Using this technique, IC-GAN can be transferred to generate images from some unseen distributions during training, by just changing the conditioning instances on the target samples, \eg, ImageNet $\rightarrow$ COCO-Stuff.

\subsection{Regularizing Label-Augmented GANs}
\citet{hou2023regularizing} uses a similar idea to the LeCam regularizer by adding a moving average regularizer on top of the label-augmented GAN.
More specifically, it pushes the prediction of the label-augmented discriminator to the moving average of the prediction of the same discriminator for the real samples.

%D3-TGAN - ACMM'23
\subsection{Data-Dependent Domain Transfer GANs with Limited (D3-TGAN)}
Data-Dependent Domain Transfer GANs with Limited (D\textsuperscript{3}-TGAN)
\cite{wu2023d3tgan} first inverts each target sample into the latent code space of the source GAN by optimizing latent code using a combination of perceptual and spatial loss.
Then, the maximum mean discrepancy (MMD) between the features of the source $G$ for inverted code and features of the adapted GAN for a random latent code is used in addition to the adversarial loss when updating the generator.
For the discriminator, the MMD between extracted features for the real (fake) images with pre-trained and adapted GAN is added to the adversarial loss during adapting the discriminator to prevent overfitting to limited data.


%\textcolor{cyan}{Transfer learning-based works will be included (the review is completed):}
%{\bf TGAN}, {\bf FreezeD}, {\bf BSA}, {\bf MineGAN}, {\bf EWC},{\bf CDC}, {\bf GANMemory}, {\bf CamGAN}, {\bf DCL}, {\bf AdAM}, {\bf \textsc{FairTL}}, and {\bf RICK}.


%\subsection{Data Augmentation Works}
%% ADA - NeurIPS'20
\subsection{Adaptive Data Augmentation (ADA)}
\citet{karras2020ada} study overfitting in GANs by training StyleGAN2 on small portions of the FFHQ dataset and observing the resulting dynamics. Results show that as training proceeds, eventually progress stops and FID starts to rise. The less training data is available, the earlier it happens.
Evaluating the discriminator output distributions for real and generated images during training show that initially, they overlap, but keep drifting apart as the discriminator becomes more confident about training images. Interestingly, the point that FID starts to rise is consistent with the loss of sufficient overlap between distributions (over-confident $D$). \citet{karras2020ada} believe that this is a strong indicator of overfitting which is evidenced further by accuracy drop (in terms of $D$'s output) measured for a separate validation set of real images from the very same distribution.
In fact, it has also previously mentioned that when $D$ is overconfident, its feedback for $G$ is no longer useful, and training starts to diverge \cite{zhang2019progressive, arjovsky2017towards}.
{\em Data augmentation} is one of the effective yet simple approaches used in discriminative learning to prevent the overfitting of deep neural networks to the training dataset. 
However, a GAN trained under similar data augmentations ---feeding augmented data directly to $D$--- learns to generate the augmented distribution \cite{Zhang2020Consistency}.
Generally, `leakage' of augmentation to generated images is highly undesirable, \eg, a noisy augmentation leads to generating noisy images even though there are no noisy images in the original training dataset.

\noindent
In \cite{karras2020ada}, a stochastic pipeline for data augmentation is proposed to prevent the leakage of the augmentation to generated images. The design of this augmentation is inspired by balanced Consistency Regularization (bCR) \cite{zhao2021improved} which is an augmentation approach proposed for training GANs with sufficient data.
Specifically, the augmentation is applied for both real and generated images during training of both $D$ and $G$.
Therefore, the $D$ only observes the augmented images (real or generated).
The main design choice to prevent leaking these augmentations to generated images by $G$ is that these augmentations are executed at a probability $p < 1$. The experimental results in \cite{karras2020ada} suggest that leaks are unlikely to happen in practice as long as $p$ remains below 0.8. In addition, by performing an exhaustive sweep over p for different augmentation categories and dataset sizes, two major conclusions are made: I) among 18 data augmentations which are grouped into 6 categories, only pixel blotting, geometric and color transforms are shown to be effective, II) The optimal value of $p$ depends on the dataset size, and a grid search is required to find this optimal value. Finally, based on these observations, an Adaptive Discriminator Augmentation (ADA) approach is proposed to find the optimal value for $p$ dynamically.

\noindent
The adaptive strategy for updating $p$ is based on two heuristics observed during the evaluation of GAN's overfitting under limited data.
Let's denote the discriminator outputs by $D_{train}$, $D_{val}$, and $D_{gen}$ for the training set, validation set, and generated images, respectively.
The analysis in \cite{karras2020ada} suggests that following the standard way (in discriminative learning \cite{santos2022avoiding}) of using a validation set to measure overfitting, when overfitting kicks in, the validation set starts behaving increasingly like the generated images. This is an easily quantifiable effect, using the following heuristic:
\begin{equation}
\label{eqn:rv_heuristic_ada}
    r_{\upsilon} = \frac{\mathbb{E}[D_{train}] - \mathbb{E}[D_{val}]}{\mathbb{E}[D_{train}] - \mathbb{E}[D_{gen}]}
\end{equation}
where $\mathbb{E}$ denotes the mean value over a batch of samples ---256 images used in practice.
Note that $r_{\upsilon}=0$ implies that $\mathbb{E}[D_{train}] = \mathbb{E}[D_{val}]$ meaning that there is no overfitting. 
Similarly, $r_{\upsilon}=1$ implies that $\mathbb{E}[D_{val}] = \mathbb{E}[D_{gen}]$ meaning the complete overfitting.
Even though the heuristic in (\ref{eqn:rv_heuristic_ada}) is helpful in assessing the overfitting, the main drawback is that it requires an additional validation set when there is a severe shortage of real data for GAN training \cite{karras2020ada}. Therefore, an additional heuristic is used in \cite{karras2020ada} which relies on the discriminator's output on training images. The observation is that when $D$ overfits training data, its outputs for real and generated images diverge symmetrically around zero. This can be quantified using the sign of $D$'s output as follows:
\begin{equation}
 \label{eqn:rt_heuristic_ada}
    r_{\tau} = \mathbb{E}[sign(D_{train})]  
\end{equation}
Similarly, $r_{\tau}=0$ means no overfitting, and $r_{\tau}=1$ denotes complete overfitting. In practice, ADA \cite{karras2020ada} only uses the $r_{\tau}$ for determining the strength of augmentation $p$, and $r_{\upsilon}$ is used only for the sanity check.
More specifically, to control augmentation strength, during training, the $p$ is initialized to zero and then adjusted every four mini-batches. If $r_{\tau}$ shows too much/little overfitting, the value of $p$ is increased/decreased by a fixed amount. In practice, $p$ is adjusted in a way to get the target value of $r_{\tau}=0.6$.
The experimental results show that ADA effectively prevents overfitting when training GAN from scratch or transferring GAN into a target domain from a pre-trained model.
During the experimental evaluation, ADA introduces a new dataset named \textsc{MetFaces}\footnote{\url{https://github.com/NVlabs/metfaces-dataset}} which is an image dataset of human faces extracted from works of art.

% cGANTransfer --- CVPR'21
\subsection{Efficient conditional GAN Transfer (cGANTransfer)} 
\citet{shahbazi2021efficient} address the efficient knowledge transfer from a pre-trained generative model in conditional GANs (cGANs).
More specifically, \cite{shahbazi2021efficient} discusses how to add new classes to a pre-trained cGAN while keeping good image generation performance on the old classes.
Inspired by \cite{noguchi2019bsa}, cGANTransfer assumes that the pre-trained $G$ is conditioned on the class labels using conditional batch normalization (BN) --meaning that each class has its own BN parameters \cite{brock2019biggan, miyato2018cgans, park2019semantic}.
Then, the explicit knowledge propagation from the old classes to new classes is enforced by defining the BN parameters to be the weighted average of the BN parameters of old classes, where the weights are learned during the adaptation as an indicator of similarity between respective classes.
In addition, knowledge sharing between all new classes is encouraged by cloning the BN parameters of the old classes and updating these parameters as the new shared base for obtaining the BN parameters for the new classes.
To improve the adaptation capability (especially for new classes that are more different from the old ones in the pre-trained cGAN), additional residual weight is learned for the BN parameters of each class.
We remark that this strategy is only applied for $G$, and the $D$ is learned by a simple fine-tuning approach. This may affect the performance of the model for image generation in the old classes. Note that cGANTransfer can only be applied to the pre-trained cGANs that use BN parameters for the conditioning on the generator.


\subsection{Consistency Regularized GAN (CR-GAN) / balanced Consistency Regularization (bCR)} 
Consistency Regularized GAN (CR-GAN) \cite{Zhang2020Consistency} is an augmentation approach which is originally proposed to stabilize GAN training and improve generation performance under sufficient data. CR-GAN enforces the output of the $D$ to be unchanged when applying several augmentations/perturbations to the real images. \citet{zhao2021improved} improves this method by applying CR to both real and generated images. The new method is termed balanced consistency regularization (bCR).
In \cite{karras2020ada, zhao2020imageaugmentation} it is shown that consistency regularization is also helpful for training GAN under limited data, but \cite{karras2020ada} further shows that since the augmentation or consistency loss is not being applied for training $G$ \cite{zhao2021improved, Zhang2020Consistency}, it opens the door for leaking the augmentation as the generator would be free to generate augmented images without being penalized for that.
\textcolor{cyan}{See whether zCR (can be found in ADA) should be included.}


%% DiffAUg - NeurIPS'20
\subsection{Differentiable Augmentation (DiffAugment)} 
During the training of GAN, the optimizer alternatively minimizes the training loss of discriminator $\mathcal{L}_D$, and the training loss of generator $\mathcal{L}_G$ with the following loss functions:
\begin{equation}
\label{eqn:diffaug_dloss}
    \mathcal{L}_D = \mathbb{E}_{x \sim p_{data}} [f_D(-D(x))] + \mathbb{E}_{z \sim p_z} [f_D(D(G(z)))]
\end{equation}
\begin{equation}
\label{eqn:diffaug_gloss}
    \mathcal{L}_G = \mathbb{E}_{z \sim p_z} [f_G(-D(G(z)))]
\end{equation}
Similar to discriminative learning, usually, during the training, the accuracy of $D$ \wrt training data keeps increasing, and the accuracy of $D$ \wrt validation data starts to decrease after a while. This is an indicator of discriminator overfitting which previously is observed for training the GAN with sufficient data (\eg training BigGAN \cite{brock2019biggan} on the large-scale ImageNet dataset). The overfitting problem of $D$ becomes even more severe when the available training data is limited. To investigate this, \citet{zhao2020diffaug} perform an experiment to track the training and validation accuracy of $D$ during training a BigGAN with $10\%$, $20\%$, and $100\%$ of CIFAR-10 dataset \cite{krizhevsky2009cifar100}.
Results show that when data becomes limited, the training accuracy of $D$ rises more quickly (to near $100\%$), and the validation accuracy degrades much faster (to lower than $30\%$). This suggests severe overfitting in $D$, which \citet{zhao2020diffaug} interprets this as memorizing the training dataset with $D$.

As data augmentation is one of the simplest approaches to mitigate the overfitting in discriminative tasks of machine learning, \citet{zhao2020diffaug} revisit the data augmentation for training GAN by considering three different variants:
\begin{itemize}
    \item {\em Augment Reals Only}. In this scenario, only real images (seen by $D$) are augmented: in (\ref{eqn:diffaug_dloss}), $f_D(-D(x))$ is replaced by $f_D(-D(\textcolor{purple}{T}(x)))$, where $\textcolor{purple}{T}$ denotes the transformation performed by data augmentation approach. The limitation of this approach is that since the data distribution is manipulated, $G$ starts to generate images with this manipulated distribution, like images with translation padding.
    
    \item {\em Augment $D$ only}. Informed by the limitation of augmenting only real images, in this setup, both real and generated images (seen by $D$) are augmented:  in (\ref{eqn:diffaug_dloss}), $f_D(-D(x))$, and $f_D(D(G(z)))$  are replaced by $f_D(-D(\textcolor{purple}{T}(x)))$, and $f_D(D(\textcolor{purple}{T}(G(z))))$, respectively.
    Note that this way of augmentation can be seen as a simplified version of bCR \cite{zhao2021improved} which is an augmentation approach proposed for training GAN with sufficient data.
    This setup diverges because of the unbalanced optimization of $D$, and $G$. As an example, for the BigGAN example, $D$ classifies the augmented images $\textcolor{purple}{T}(x)$, and $\textcolor{purple}{T}(G(z))$ with high accuracy ($>90\%$), but has less understanding about generated images ($<10\%$ classification accuracy for $G(z)$).

    \item {\em Differentiable Augmentation}. Due to limitations in the two previous approaches, finally, \citet{zhao2020diffaug} propose to augment both real and generated images when updating $D$, and $G$, resulting in the following loss functions:
    \begin{equation}
    \mathcal{L}_D = \mathbb{E}_{x \sim p_{data}} [f_D(-D(\textcolor{purple}{T}(x)))] + \mathbb{E}_{z \sim p_z} [f_D(D(\textcolor{purple}{T}(G(z))))]
    \end{equation}
    \begin{equation}
    \mathcal{L}_G = \mathbb{E}_{z \sim p_z} [f_G(-D(\textcolor{purple}{T}(G(z))))]
    \end{equation}
    Note that since $\textcolor{purple}{T}$ is on the path of propagating the gradient to $G$, it should be differentiable, named DiffAugmentation.
\end{itemize}
\noindent
After finding the best configuration to apply the augmentation, the experimental results in \cite{zhao2020diffaug} show that the best augmentation approaches for this configuration are: {\em Translation} (within [-1/8, 1/8] of the image size, padded with zeros), {\em Cutout} \cite{devries2017improved} (masking with a random square of half image size), and {\em Color} (including random brightness within [-0.5,0.5], contrast within [0.5,1.5], and saturation within [0,2]).
During experimental comparisons, the baselines are augmented with a random horizontal flip which shows to be beneficial in most cases.
DiffAugmentation is also shown to be orthogonal to transfer-learning-based approaches by bringing additional improvements when used with these approaches.
Note that other simple solutions to prevent overfitting in deep neural networks are regularization, and decreasing the network capacity. These solutions are also considered for both BigGAN and StyleGAN2 in \cite{zhao2020diffaug}, showing that these approaches (decreasing channel size; enhancing the impact of $R_1$ regularization) just bring a limited enhancement compared to the data augmentation for training GANs under limited data.
Note that this could be because of the naive way of implementing these ideas because future works in the literature show that using both regularizers and decreasing capacity/making capacity dynamic can largely improve training GANs under limited data.


\subsection{Data Augmentation Optimized for GAN (DAG)}
\citet{tran2021dag} proposes a theoretical analysis to show that Jensen-Shannon (JS) divergence between two distributions is invariant under differentiable and invertible transformations.
This means that using an invertible transformation as augmentation (\eg, rotation) the JS preserving can be guaranteed. \textcolor{cyan}{Some additional info about JS divergence in the original GAN, and under augmentation could be added here.}
Inspired by this, \cite{tran2021dag} proposes to augment both real and generated images prior to feeding them to $D$. However, since sharing $D$ for all samples doesn't preserve the JS divergence, multiple $D$'s (one for non-augmented samples, and one for each augmentation) are used during training GAN.
The major limitation of using multiple separate discriminators is that each $D$ may overfit its own dataset. 
To resolve this issue, a weight-sharing mechanism is proposed as a regularizer to improve the generalization performance of the discriminators.
The proposed framework ---called Data Augmentation optimized for GAN (DAG)--- is shown to be beneficial for training unconditional GAN, conditional GAN, and Image-to-Image translation in both sufficient-data and limited-data regimes.


\subsection{Image Augmentation for GAN Training (IAG)} 
Similar to ADA \cite{karras2020ada}, DAG \cite{tran2021dag}, and DiffAugment \cite{zhao2020diffaug}, image Augmentation for GAN (IAG) training \cite{zhao2020imageaugmentation}, discusses that only augmenting real images can degrade image generation performance, and both real and fake images are required to be augmented before feeding to $D$. 
The results of applying different augmentation techniques show that spatial augmentations (\eg, zooming in/out) are more effective than visual augmentations (\eg, brightness change), and some visual augmentations like adding instance noise can degrade image generation performance even though stabilizing the training process.
From the perspective of data distribution, the difficulty of training GAN is that the distributions of the real and fake images are very concentrated, and their support does not overlap \cite{arjovsky2017towards, sonderby2017amortised}. 
The discussion in \cite{zhao2020imageaugmentation} suggests that augmentation increases the overlap between the distribution of real and fake images and therefore improves image generation quality.
\citet{zhao2020imageaugmentation} also show that augmenting real and fake images can be combined with consistency regularization to further improve the image generation quality by GAN.
\textcolor{cyan}{Consistency regularization forces the score of $D$ to be the same for a (real/fake) under different augmentation. Conceptually, it is a similar goal to augment both real and fake images, but the question is how these two approaches are complementary and can enhance together.}
In addition, inspired by SimCLR \cite{chen2020simclr}, they have proposed to apply a simple contrastive learning approach when training $D$ which is a related approach to augmentation as different views are just created by applying the augmentation.
Then they have shown that this approach can be combined with consistency regularization to further improve image generation performance.
\textcolor{cyan}{Similarly, the interesting thing is that different augmentation-based approaches can be complementary to each other. Finding how different knowledge is being used with different types of augmentation-based learning signals could be an interesting section of this survey.}



% D2C - NeurIPS'21
\subsection{Diffusion-Decoding models with Contrastive Representation (D2C)}
Diffusion-Decoding with contrastive Representation (D2C) \cite{sinha2021d2c} aims to improve the sample generation of the VAEs with improving the latent code using denoising techniques.
More specifically, a diffusion model is trained to denoise the latent code and output a clean latent code which is then used by the VAE decoder to generate an image with improved quality.
Additionally, a classifier is learned over latent space based on the label information to capture the relation of a latent region with each label, and it is used together with the diffusion model to fetch clean latent codes for a determined label / class.
The proposed D2C is shown to be beneficial for training the VAE under limited data.


% Label-Augmentation - NeurIPS'21
\subsection{Self-supervised GANs with Label Augmentation}
Recall that DAG \cite{tran2021dag} uses multiple discriminators, each of which performs the real/fake classification under a specific data transformation. \citet{hou2021labelaugmentation} extends this idea by merging all these discriminators into one discriminator and augmenting the labels of the task that $D$ should handle. 
More specifically, instead of only handling real/ fake classification, the discriminator performs multi-class classification of $(l,k)$, where $l \in \{ Real, Fake\}$, and $k=1,..., K$ denotes the index of the transformation $T_k(.)$ applied on both real and fake data.
By performing these two classification tasks simultaneously, a more robust $D$ is learned which can give more meaningful feedback to the $G$ for image generation under both large-scale and limited data scenarios.

% DecieveD - NeurIPS'21
\subsection{Adaptive Pseudo Augmentation (APA)} 
Similar to ADA \cite{karras2020ada}, Adaptive Pseudo Augmentation (APA) \cite{jiang2021deceive} uses a heuristic to adaptively augment the limited data during training GAN. However, instead of using augmentation transformation, APA feeds the generated images by $G$ as pseudo-real data to enlarge the real dataset.
The rationale behind this design is that under limited data, $D$ overfits real images by being overconfident in real-fake discrimination ---observed by increasing the divergence in $D$'s score for real and fake images. 
Blindly presenting the fake images as reals to $D$ can weaken the discriminator's ability on performing its fundamental task of real-fake classification.
To prevent this negative effect, in each training iteration, pseudo-augmentation is applied with the probability $p$ and is skipped with probability $1-p$.
The value of $p$ is determined adaptively based on the training dynamics.
Specifically, the expected value of the sign of the discriminator's logit for real samples 
\begin{equation}
\lambda_r = \mathbb{E} \{ sign[logit(D(x))] \}
\end{equation}
is used as a heuristic to measure the $D$'s overfitting, where $\lambda_r = 0$ represents no overfitting, and $\lambda_r = 1$ means complete overfitting.
Analysis in \cite{jiang2021deceive} shows that similar heuristics on fake samples, or the average on real and fake samples can also be used as an indicator of overfitting.
After defining the heuristic $\lambda_r$, a threshold $t$ is set, and $p$ is initialized to zero. Then, during training, $p$ is increased/decreased if $\lambda_r$ is larger/smaller than $t$.
The theoretical analysis in \cite{jiang2021deceive} shows that under the mild assumption of $\alpha$ being the expected strength that approximates the effect of dynamic adjustment, for a fixed G, the optimal discriminator $D^*$ for APA is: 
\begin{equation}
 D^*_G(x) = \frac{(1-\alpha)p_{data}(x) + \alpha p_g(x)}{(1-\alpha)p_{data}(x) + (1+\alpha) p_g(x)}   
\end{equation}
Then, it is shown that for the optimal $D^*$, the generation process of APA can be considered as minimizing the JS divergence between smoothed data distribution and generated distribution:
\begin{equation}
    \mathcal{V}(G, D^*) = -log4 + 2 \cdot JS(\{(1-\alpha)p_{data} + \alpha p_g\} \| p_g)
\end{equation}
APA is shown to be beneficial for both limited data and sufficient data regimes, and it is shown to be complementary to other GAN augmentation approaches like ADA \cite{karras2020ada}.


%AdvAug - NeurIPS'21
\subsection{Adversarial Augmentation (AdvAug)}
\citet{chen2021advaug} make two major contributions to training GAN under limited data. First, inspired by the lottery ticket hypothesis (LTH), \cite{chen2021advaug} show that under limited data using a sparse subnetwork can give better image generation performance than the original dense network. More specifically, LTH \cite{frankle2019lotteryticket} shows the existence of independently trainable sparse subnetworks that can match or even surpass the performance of the dense network.
The idea of LTH is extended to generative learning in \cite{chen2021ganslottery, kalibhat2021winning} who validated the existence of winning tickets when training GAN in the min-max game. However, \cite{chen2021advaug} is the first work that shows using the winning ticket can improve image generation compared to the original dense GAN structure.

\noindent
Then, \cite{chen2021advaug} proposes an adversarial augmentation (AdvAug) to further improve the performance of the GAN ticket under limited data. More specifically, AdvAug separately computes the adversarial perturbation $\delta$ for the feature maps of the discriminator and generator using the projected gradient descent (PGD) \cite{madry2018towards}. Denoting the discriminator as $D = D_2 \circ D_1$, the adversarial augmentation is applied on the intermediate feature maps ($D_1$) of both real and generated images, resulting in $D_{1}(x) + {\delta}$, and $D_{1}(G(z)) + {\delta}$. The adversarial loss is then added to the loss function of $D$ during GAN training to maximize the score of the perturbed real image and minimize the score of the perturbed generated image. The adversarial loss can be depicted as:
\begin{equation}
    \mathcal{L}_{D}^{adv} \coloneqq \max_{\| \delta \|_{\infty} < \epsilon} \mathbb{E}_{x \sim p_{data}} [f_{D}(-D_2(D_1(x)+\delta))] 
    +
    \max_{\| \hat{\delta} \|_{\infty} < \epsilon} \mathbb{E}_{z \sim p_{z}} [f_{D}(D_2(D_1(G(z))+\hat{\delta}))] 
\end{equation}
Similarly, for $G = G_2 \circ G_1$, the adversarial perturbation is added to $G_1(z)$ and the corresponding adversarial loss is added to the generator loss during training.
As AdvAug is performed on the feature level, it is shown to be complementary to image-level augmentations like ADA \cite{karras2020ada} and DiffAug \cite{zhao2020diffaug} and can bring further improvements when applied together with these approaches.


\subsection{Diffusion-GAN: Training GANs with Diffusion}
Diffusion-GAN \cite{wang2023diffusiongan} applies the gradual diffusion process ---used in the training process of the DMs--- to both real and fake images during the training of GAN to prevent overfitting $D$ to training data.
The idea is similar to previous augmentation approaches for GAN (\eg, ADA \cite{karras2020ada}, and DAG \cite{tran2021dag}) where both real and generated images are augmented, however, the difference is that the strength of augmentation (added noise in the diffusion process) is being gradually increased in \cite{wang2023diffusiongan}.
This means that the hardness of the bi-classification task performed by $D$ is being increased as training goes on.
Note that based on the simplified diffusion modeling, the diffusion operation is differentiable, meaning that the gradients can be backpropagated to the $G$.
The theoretical analysis in \cite{wang2023diffusiongan} shows that minimizing the JS-divergence between perturbed versions of the real data and generated distributions equals minimizing the JS-divergence between the original distributions of the real and generated data. 
In addition, an adaptive diffusion step size is proposed that considers the amount of overfitting in $D$ when determining the maximum steps for the diffusion process.


% PatchDiffusion - arXiv'23
\subsection{PatchDiffusion: Faster and More Data-Efficient Training of Diffusion Models}
\citet{wang2023patchdiffusion} propose a simple patch-wise training framework for diffusion models to improve the data efficiency and decrease the training time of diffusion models.
This framework augments the training samples by sampling patches with random locations and random sizes alongside the full image during the training of a diffusion model. 
The denoising score function \cite{karras2022elucidating} is conditioned on the patch size and the location information of the patches. 
In addition, the coordinate of the full image is normalized to $[-1,1]$, and the normalized coordinate information of each patch is appended as additional channels during training.
PatchDiffusion improves the image generation performance of the DMs for both large-scale datasets and limited data ($\sim$5K) scenarios.

% ECCV'22
\subsection{Any-Resolution GAN Training}
PatchDiffusion \cite{wang2023patchdiffusion} is inspired by \cite{chai2022anyresolution} that proposes a patch-level training framework to generate images in any resolution.
More specifically, \citet{chai2022anyresolution} proposes to train a generator jointly on the low-resolution dataset for learning the global structure of the images, and on patches from varied-size datasets to learn details.
Even though not proposed for the limited data scenario, \cite{chai2022anyresolution} removes the need for large-scale high-resolution images to generate images with the same resolution.


%SinGAN - ICCV'19
\subsection{Single Image GAN (SinGAN)}
In \cite{shaham2019singan}, the problem of training a GAN from scratch using only one natural image is addressed. Trained GAN ---called Single Image GAN (SinGAN)--- can generate plausible and novel compositions of a scene (reference image) that have a similar visual context to the reference image. 
The main idea is that the internal distribution of the patches within an image provides a powerful prior for training a generative model.
Therefore, instead of using a set of images within a dataset, the patches within a single image are used as training data, and the generative model is trained to capture the internal distribution of these patches. This goal is achieved by training a pyramid of GANs to learn the distribution of patches on different scales. More specifically, a pyramid of generators $\{G_0, \dots, G_N \}$ are trained against a pyramid of real images $\{x_0, \dots, x_N \}$, where $x_n$ is a downsampled version of input image $x$ by a factor of $r^n$. The generator at scale $n$ uses random noise $z_n$ and upsampled version of the generated image from the lower resolution ($\tilde{x}_{n+1}$) to generate images:
\begin{equation}
    \label{eqn:singan}
    \tilde{x}_{n} = G_n(z_n, (\tilde{x}_{n+1})\uparrow^{r_{n}})
\end{equation}
Additionally, $D_n$ compares the $\tilde{x}_{n}$ and $x_{n}$ in patch-level for real-fake classification.
Note that for $n=N$ (lowest resolution), $G_N$ only uses noise as input.
An additional reconstruction loss is added to ensure the generator makes good use of $z$ during image generation.
After training the generator on a single image, different editing tasks can be performed by inserting manually edited images as $\tilde{x}_{n}$ in lower scales.
To evaluate the performance, in addition to Inception Score (IC), they propose Single Image FID (SIFID) which computes FID between the internal distribution of deep features at CNN's output.

%{\bf InGAN.}
We remark that Internal GAN (InGAN) \cite{shocher2019ingan} is a concurrent work with SinGAN that aims to address training a GAN using a single image by capturing the internal patch distribution of the reference image. However, InGAN is an editing scheme (image-to-image generation) model that uses a UNet-Shaped \cite{ronneberger2015unet} generator and only changes the size or aspect ratio of the input with keeping the exact information of the input image.

% ConSinGAN -- WACV'21
\subsection{Concurrent Single Image GAN (ConSinGAN)}
In \cite{hinz2021consingan}, through analyzing the performance of SinGAN \cite{shaham2019singan}, some good practices are discussed for training GANs from scratch using one natural image by proposing three major improvements. 
The most important one is changing the multi-scale training scheme. 
Instead of using separate generators for each scale, ConSinGAN stacks the new layers for a bigger scale on top of the previous layers used for a smaller scale. 
These weights are connected using an {\em `Upsampling + Noise'} operation where upsampling increases the image scale to the current one and noise is added to increase the generation diversity.
The upscaled feature is also added to the output of the newly added layers using a skip connection \cite{he2016resnet} to enforce the newly added layers to learn the residual features.
In contrast to SinGAN which just trains parameters of each scale at a time while keeping previous ones frozen, ConSinGAN trains layers from multiple scales  concurrently whereas the layers from previous scales are trained with a smaller learning rate.
Similar to SinGAN in each scale, the real/fake classification task is performed using a downsampled version of the reference image, however, logarithmic downsampling is used (instead of geometric in \cite{shaham2019singan}) to give more attention to lower scales of the image.
Finally, when used for editing applications (\eg, harmonization), the generator is trained in a task-specific manner by using an augmented real image that resembles the editing task.



%One-Shot GAN -- CVPR'21 workshop
\subsection{One-Shot GAN}
One-Shot GAN \cite{sushko2021oneshotgan} extends the setup of SinGAN \cite{shaham2019singan} to generate images from one image or on video (using the frames within the video).
Similar to SinGAN, the aim of \cite{sushko2021oneshotgan} is to generate novel composition of a reference scene. For this, One-Shot GAN hypothesizes that the generator should learn objects' appearance and how to combine them. This is implemented using multiple paths in the discriminator. 
Specifically, within the discriminator, after extracting low-level features, the loss $\mathcal{L}_{\texttt{low-level}}$ is defined on these features. Then, on top of these low-level features, two different types of losses are defined: i) $\mathcal{L}_{\texttt{content}}$ which aims to learn {\em content} by aggregating spatial information through global average pooling, ii) $\mathcal{L}_{\texttt{layout}}$ which aims to obtain {\em layout} using aggregation via $1 \times 1$ convolution.
All of these three losses are trained in an adversarial manner. In addition, a regularizer is added to enforce diverse image generation by pushing away the features of generated images with different seeds.



% LeCam - CVPR'21
\subsection{Regularizing GAN with LeCam-divergence}
\citet{tseng2021lecam} proposes a regularizer to improve the training stability and mitigate the overfitting to real images when training GANs under limited data. Specifically, two exponential moving average values are used to track the $D$'s prediction for real ---denoted by $\alpha_R$--- and generated ---denoted by $\alpha_F$--- images during training.
Then they propose to regularize the distance between the $D$'s prediction for real (fake) images and $\alpha_F$ ($\alpha_R$) by adding the following term to $D$'s optimization objective:
\begin{equation}
\label{eqn:lecam_regularizer}
    R_{LC} = \mathbb{E}_{x \sim p_{data}} [\| D(x) - \alpha_F \|^2] +
    \mathbb{E}_{z \sim p_z} [\| D(G(z)) - \alpha_R \|^2]
\end{equation}
Even though $R_{LC}$ in Eqn.\ref{eqn:lecam_regularizer} looks counter-intuitive since it pushes $D$ to mix the prediction for real and fake images, the theoretical analysis in \cite{tseng2021lecam} shows that adding this regularizer to WGAN \cite{arjovsky2017wasserstein} (BigGAN\cite{brock2019biggan}) enforces it to minimize the LeCam-divergence.
Then, they empirically show that LeCam-divergence is a more robust function for training GAN under limited data.
The experimental results show that the LeCam regularizer enhances the performance for both sufficient and limited data scenarios, and also complements the performance of the data augmentation approaches proposed for training GAN with limited data.
Moreover, the analysis on reducing the capacity of $G$ shows that the lower capacity of $G$ can improve image generation when limited data is available (similar to the idea of FastGAN), and LeCam is more beneficial for high-capacity networks.



% InsGen - NeurIPS'21
\subsection{Data-Efficient Instance Generation (InsGen)}
In a data-limited regime, $D$ is not learning proper/generalizable features because of overfitting to real images. \citet{yang2021insgen} aims to improve representation learned by $D$ through introducing a pretext task.
Specifically, inspired by the recent success of contrastive learning for self-supervised learning, InsGen applies a similar idea during training GAN under limited data.
Contrastive learning can train a model with a powerful discriminative representation in an unsupervised manner (without annotated data).
The rationale behind contrastive learning is to "label" each sample as an individual class, \ie, instance discrimination.
Given an image $x$, contrastive learning  generates two views (through different augmentations) as the query $x_q$ and the key $x_{k_+}$. The query and key are treated as positive pairs, and all "views" from other images, $\{x_{k_i} \}_{i=1}^{N}$ are treated as negative pairs \wrt query.
Then, the objective is to learn a representation that maps positive pairs together and pushes the negative ones away. Therefore, a pretext task of $(N+1)$-way classification can be designed to learn the model --termed InfoNCE loss in \cite{oord2018infonce}:
\begin{equation}
    v_q = F(x_q), \quad v_{k_+} = F(x_{k_+}), \quad v_{k_i} = F(x_{k_i}); \: i=1,\dots,N
\end{equation}
\begin{equation}
    \mathcal{L}_{\texttt{InfoNCE}} = - \log \frac{exp(\phi(v_q)^T\phi(v_{k_+})/\tau)}{\sum_{i=0}^{N} exp(\phi(v_q)^T\phi(v_{k_i})/\tau)}
\end{equation}
where $F(.)$ is the backbone used for feature extraction, $\phi(.)$ is the head to project features into a unit sphere, and $\tau$ is the temperature parameter.
Drawing inspiration from contrastive learning, InsGen proposes four modules to improve representations learned by the discriminator of the GAN under limited data:
\begin{itemize}
    \item {\em Distinguishing real images:} Similar to contrastive learning, an instance discrimination loss is added to the default real-fake detection task of the discriminator. Assuming that vanilla $D$ consists of a backbone $f(.)$ and a classification head $\phi^{domain}(.)$, the instance discrimination of real images is done using the same backbone and adding an extra head $\phi^{r}(.)$ for the new task.
    \item {\em Distinguishing fake images:} As the number of real images is limited, instance discrimination is also applied to fake images --which are unlimited in number-- using a separate head $\phi^{f}(.)$ to compensate for the distribution shift between real and fake images and also prevent the evolving distribution of the fake images to harm learning  $\phi^{r}(.)$.
    \item {\em Noise perturbation:} To make instance discrimination of the fake images more challenging, and therefore learning a more discriminative representation by $D$, InsGen makes use of the continuity of the latent space of GANs \cite{radford2015unsupervised} during constructing views by fake images. Specifically, for a query generated with some random noise $x^{'}_{q} = \mathcal{T}_{q}[G(z_q)]$ the corresponding key is generated by adding a small perturbation $\epsilon$ (sampled from a Gaussian noise but much smaller than $z$ in terms of magnitude) to the same noise used for query generation: $x^{'}_{k_+} = \mathcal{T}_{k_+}[G(z_q+\epsilon)]$. Note that $\mathcal{T}_{q}(.)$ and $\mathcal{T}_{k_+}(.)$ denote two different augmentations. This enforces the discriminator to be robust against small perturbations in the generated image.
    \item Finally, the discrimination loss on fake samples is also looped back to $G$ to enforce the generation of diverse samples.
\end{itemize}
To learn each task head for instance discrimination, following MoCo-v2 \cite{he2020momentum, chen2020improved}, an extra queue is employed for each head to store the sample features for the computational cost.
In addition, $D$ is updated as a momentum encoder using the moving average scheme. To evaluate the better representation learning by the discriminator, the $D$'s output for real and fake images is compared with the baseline (StyleGAN2-ADA) where the discriminator learned under the proposed method gives better values (a higher value for real images and a less value for fake images).



%% FastGAN - ICLR'21
\subsection{FastGAN}
As the high capacity of current SOT GANs like StyleGAN2 \cite{karras2020analyzing} increases the risk of overfitting or mode collapse under limited data, \citet{liu2021fastgan} proposes to use a lightweight GAN structure ---called FastGAN--- to decrease this risk for high-resolution (up to $1024 \times 1024$) image generation with limited data.
For efficient training of this lightweight structure under limited data, the design goal is to have a $G$ that learns fast, and a powerful enough $D$ that continuously provides valuable feedback for $G$. 
Specifically, $G$ consists of upsampling layers (Nearest Neighbor upsampling followed by a Conv layer) which consecutively increase image resolution.
In order to have a better gradient flow between these layers, inspired by skip connection design \cite{he2016resnet, he2016identity}, Skip-Layer Excitation (SLE) module is proposed which fuses features from the different resolutions by multiplying high-resolution features $\hat{x}_{high}$ with processed low-resolution ones $\hat{x}_{low}$ as follows:
\begin{equation}
    \hat{x}_{high}^{'} = \mathcal{F}(\hat{x}_{low}) \odot \hat{x}_{high}
\end{equation}
where $\mathcal{F}$ indicates a set of Conv layers. Note that different from the skip connection used in ResNet \cite{he2016resnet}, the SLE module is applied between features with different resolutions (\eg, $8\times8$ and $128\times128$), and uses multiplication to save computational cost. SLE also resembles the Squeeze-and-Excitation module \cite{hu2018squeeze} with the difference that \cite{hu2018squeeze} operates within only one featuremap. 

\noindent
To enhance $D$'s performance in providing useful feedback for the generator, a self-supervised approach is used to train $D$. Specifically, by examining the different design choices of self-supervised learning, the auto-encoder-based design has been shown to perform better.
More specifically, in addition to the primary bi-classification task of the $D$, a secondary task is considered where $D$ is treated as an encoder and is trained with two small decoders. 
This additional auto-encoding task enforces $D$ to extract image features that decoders can give good reconstructions. For this task, the decoders and $D$ are optimized by a reconstruction loss only on real images $x$:
\begin{equation}
    \mathcal{L}_{\texttt{recons}} = \mathbb{E}_{\mathbf{f} \sim D_{enc}(x);\; x \sim p_{data}} \{ \| \mathcal{G}(\mathbf{f}) - T(x) \| \}
\end{equation}
where $\mathbf{f}$ denotes intermediate feature-maps reconstructed by $D$, $T$ denotes pre-processing like down-sampling or crop used on real and generated images during training, and $\mathcal{G}$ contains the same processing with decoding module.
Using these two simple techniques, FastGAN is able to produce better images than SOTA baseline StyleGAN2 under limited data in various resolutions (from $256\times256$ to $1024\times1024$) and using extremely lower computational complexity.
Ablation studies in \cite{liu2021fastgan} show that the biggest contribution to the performance of the FastGAN comes from the $D$, showing the vital importance of the discriminator on the GAN structure.
In addition, one intuition behind performance improvement brought by $D$ is that auto-encoding forces $D$ to pay attention to more areas of the input image and extract more comprehensive features from the images. As we will discuss later, a similar intuition is used on MaskedGAN \cite{huang2022maskedgan}, where they mask real images to prevent $D$ from learning trivial solutions and enforce it on learning more hard and comprehensive features.


% ProtoGAN - Information Sciences'23
\subsection{Prototypical GAN (ProtoGAN)} 
Prototypical GAN (ProtoGAN) \cite{yang2023protogan} aims to improve the fidelity and diversity of the FastGAN under limited data inspired by the recent success of the learning prototypes in few-shot classification \cite{snell2017prototypical} and few-shot semantic segmentation \cite{wang2019panet}.
ProtoGAN has two main modules: prototype alignment for increasing the fidelity of the generated images, and diversity loss to improve the generation diversity.
Specifically, building on top of FastGAN \cite{liu2021fastgan}, ProGAN adds a prototype alignment loss. It first extracts the features of the batch of real and fake images using the penultimate layer of the discriminator denoted as $F_r$ and $F_f$.
Then the prototype of the real images and fake images are calculated by simply taking the mean value of the $F_r$ and $F_f$.
As using a batch of images ($N=8$ in ProtoGAN) in each iteration may not be an accurate representation of the prototype, a momentum update is proposed for calculating the prototype of the real images to include the feature maps from all available real images. A feature-matching loss is also considered to enforce the similarity of the features for generated images and real images in each batch.
Finally, to improve generation diversity, the variance loss is included to increase the variance of the generated images in the spatial domain:
\begin{equation}
    \mathcal{L}_{var} = \mathbb{E} \{ G(z_i) - \overline{G}(z) \}
\end{equation}
where $\overline{G}(z)$ is the mean of the generated images for a batch of randomly sampled noises $z$.


% ProjectedGAN - NeurIPS'21
\subsection{Projected GANs Converge Faster (ProjectedGAN)}
\citet{sauer2021projectedgan} propose to project the real and generated images into the feature space of a pre-trained vision model to enhance $D$'s performance in discriminating real and fake images.
In \citet{sauer2021projectedgan} it has been shown that na\"ive way of applying this idea ---feeding extracted features of the real and fake images to the standard $D$ in GAN--- does not lead to SOTA results as in this case $D$ dominates the two-player game, resulting in vanishing gradient for $G$ \cite{arjovsky2017towards}.
Then, ProjectedGAN proposes two modules to harness the representative power of pre-trained vision models for the real/fake discrimination task during GAN training. 

The first module is the feature pyramids where instead of only using the penultimate layer, the output from multiple layers is extracted to be used in the real-fake classification task.
The rationale behind this design is that by feeding featuremaps with different scales, more information about the input signal (real/generated image) is preserved.
Then, for each of the extracted feature maps, a separate discriminator is used to process that feature map \wrt discriminative task resulting in multi-scale discriminators.
The second module that aims to facilitate the usage of the extracted features is {\em random projection}. Based on the provided experimental results, the features at deeper layers are significantly harder to cover with the generator. Therefore, they propose to use a random projection to dilute the features and encourage the discriminator to focus on a subset of the features.

These two modules are deployed in two different schemes. Cross-channel mixing (CCM) uses a $1\times 1$ convolution as a generalization of the permutation \cite{kingma2018glow} for random projection. Note that this $1\times 1$ convolution layer is not trained during GAN training. Specifically, it is first randomly initialized using Kaiming initialization \cite{he2015delving} and then this random value is kept fixed through training and inference as random projection.
The second design termed cross-scale mixing (CSM) is built on top of CCM where it adds cross-scale information flow by adding a random $1\times 1$ convolution with bilinear upsampling within each consecutive feature map used in CCM.

In experiments, different pre-trained models are used as feature extractors including the ResNet family \cite{he2016resnet}, EfficientNet family \cite{tan2019efficientnet}, R50-CLIP
\cite{radford2021CLIP}, ViT \cite{dosovitskiy2020image} and DeiT \cite{touvron2021training}. Results suggest that in general, EfficientNet-Lite induces the best performance for ProjectedGANs.
The experimental results suggest that when combined with FastGAN, ProjectedGAN converges faster and achieves a steady performance gain (in terms of reduction in FID) in a wide range of datasets and in both sufficient and data-limited regimes.



%% MoCA - ICLR'22
\subsection{Memory Concept Attention (MoCA)} 
\citet{li2022moca} proposes to 
enhance $G$ using some memory priors to improve the image generation quality under limited data.
The idea is inspired by recent discoveries about the existence of complex, diverse, and super-sparse neural codes in macaque monkeys' primary visual cortex (V1).
The memory priors are then constructed and utilized by $G$ to resemble this phenomenon during image generation. 
In a nutshell, for each feature map of $G$ denoted by $A \in \mathbb{R}^{n\times c\times h\times w}$, MoCA \cite{li2022moca} generates a corresponding attention-based feature $H \in \mathbb{R}^{n\times c\times h\times w}$ which is then used to produce the modulated feature map $\hat{A} \in \mathbb{R}^{n\times c\times h\times w}$. 
Before starting the attention procedure to extract $H$, each featuremap $A$ is transformed into a lower-dimensional space using a set of $1\times1$ convolutions $\theta(.)$, $\phi(.)$, and $\psi(.)$, where $\{\theta(.), \phi(.), \psi(.)\}\in \mathbb{R}^{n \times \tilde{c} \times h \times w}$.
Then, two different attention mechanisms are utilized to generate $H$: I) a memory attention mechanism is used to attend to the current feature map based on memory prior, and II) a self-attention mechanism is used to attend to the current pixel location based on its neighbors.
In what follows, first, we discuss the construction of memory prior, and then based on that the details of the attention modules will be discussed.

\noindent
The memory prior is implemented using a set of semantic cells $\{K_i \}_{i=1}^{M}$. 
Each semantic cell $K_i$ is responsible to encode a concept, \eg a semantic cell could be related to rail tracks when training GAN on the "Train" category of the MSCOCO dataset \cite{lin2014microsoft}. 
For each semantic cell, there are $T$ different prototype cells $\{E_j^{(i)} \}_{j=1}^{T}$ stored in the memory cell, each of which captures different types of information about that concept resulting in more diversity. 
The average value of these prototype cells is used to represent the semantic cell: $K_i = \sum_{j=1}^{T} E_j^{(i)}/T$, where $E_j^{(i)}$ and $K_i$ both $\in \mathbb{R}^{\tilde{c}}$.
The prototype cells $E_j^{(i)}$ are updated during the training of GAN using generated features by $G$. 
More specifically, in iteration $t$ of training GAN, each hyper-column of $A$ (denoted by $A_{ij} \in \mathbb{R}^c$) is mapped to another feature space using momentum context encoder $\widetilde{\phi}(.)$. Then the closest semantic cell is retrieved based on the distance of $\widetilde{\phi}(A_{ij})$ and $K_i$s. Finally, $\widetilde{\phi}(A_{ij})$ is replaced randomly with one of the previous prototypes (updated in previous iteration $t-1$). Once all of the prototypes are updated in the current iteration, the semantic cell values $K_i$s are also updated accordingly.
Note that the momentum context encoder is inspired by the idea of MoCo \cite{he2020momentum} which follows a momentum update to accumulate information beyond the current training batch.


\noindent
After describing the construction of memory prior, we discuss the details of the attention mechanism. 
For each hyper-column of the activation function $\mathbf{a} \in \mathbb{R}^{\tilde{c}}$, first, the closest semantic cell $K_i$ is selected and all corresponding $\mathbf{E}^{(i)} \in \mathbb{R}^{\tilde{c}\times T}$ prototypes are retrieved. The similarity between this hyper-column and prototypes is calculated as $\mathbf{s}=\mathbf{E}^{(i)}\mathbf{a}$, which is then passed into a softmax operator which finally gives attention weights $\boldsymbol{\beta}$ of each memory prototype for the hyper-column. These attention weights are used to retrieve the information from memory for the current hyper-column as follows: $\mathbf{h}_m = \boldsymbol{\beta}\mathbf{E}^{(i)}$, where $\mathbf{h}_m \in \mathbb{R}^{\tilde{c}}$.
This process is repeated for each hyper-column and each generated sample in the batch to obtain the memory attention features $\mathbf{H}_m \in \mathbb{R}^{n \times \tilde{c} \times h \times w}$.
In addition to memory attention, inspired by the recent success of self-attention in capturing non-local dependency \cite{zhang2019self}, spatial contextual attention is also applied to generated feature maps. Specifically, an affinity map is firstly computed between $\theta(A)$ and $\phi(A)$ as $\mathbf{S}=[\theta(A)]^T \phi(A)$. Then, each row of the $\mathbf{S}$ is normalized by softmax to get attention weights $\hat{\mathbf{S}}$, which is then multiplied by $\phi(A)$ to get spatial context modulation tensor $\mathbf{H}_s \in \mathbb{R}^{n \times \tilde{c} \times h \times w}$. The final modulation tensor is computed by adding the modulation tensors obtained in two parallel paths: $\mathbf{H} = \mathbf{H}_m + \mathbf{H}_s$. This modulation tensor is used together with a $1\times 1$ convolution to compute the modulate feature map: $\hat{A}=\gamma O(\mathbf{H})+A$.
Note that as MoCA just works on the $G$, it is orthogonal to other approaches that enhance $D$, like ADA, DiffAug, and DynamicD.


% Training Class-conditional GANs with Limited Data - ICLR'22
\subsection{Training cGANs with Limited Data: Collapse by Conditioning (CbC)}
\citet{shahbazi2022collapse} show that under limited data setup, where an unconditional GAN can generate satisfactory performance, training the conditional GANs (cGANs) results in mode collapse. 
To mitigate this issue a training procedure is proposed to leverage the stability of the unconditional GANs. Specifically, training starts from an unconditional GAN (StyleGAN2-ADA) and slowly is transitioned to a cGAN using a transition function $\lambda_t \geq 0$.
This transition function is defined as a simple linear function that reaches from 0 to 1, and the transition starts in $T_s$, and ends in $T_e$:
\begin{equation}
    \lambda_t = \min (\max(\frac{t-T_s}{T_e-T_s},0),1)
\end{equation}
where $t$ indicates training iteration.
Considering the conditioning variable as $c$, this transition is implemented in $G$ as $G(z,c,\lambda_t)=G(S(z)+\lambda_t.E(c))$, with $S$ and $E$ as neural networks that transform the latent code and the conditioning variable.
This design enables using the same structure for $G$ in both conditional and unconditional training scenarios.
For the discriminator, the conditioning is performed by matching the feature maps of the generated image with the target class embedding through the dot product operator which provides the soft output for class probabilities. The corresponding conditional loss is multiplied by transition function $\lambda_t$ to enable transitioning the same $D$ from unconditional to conditional setup.
The experimental results show that under limited data, the proposed transitioning scheme works better than both unconditional and conditional GAN. 
These changes in structure during training and therefore in dynamics of training are also observed in DynamicD \cite{yang2022dynamicd}.


% Ensembling of-the-shelf models for GAN training - CVPR'22
\subsection{Ensembling of-the-shelf Vision Models}
In \cite{kumari2022ensembling}, it has been shown that knowledge in large vision models can decrease the training time of GAN and increase the image generation quality when used in an ensemble of discriminators.
More specifically, an ensemble of the original discriminator $D$ and additional discriminators $\{ \hat{D}_n \}_{n=1}^{N}$ is created to perform the binary real/fake image classification task.
The additional discriminators $\{ \hat{D}_n \}_{n=1}^{N}$ are trained based on a set of pre-trained feature extractors $\mathcal{F} = \{ F_n \}_{n=1}^{N}$ (trained for tackling different vision tasks), and by adding $C_n$ as a small trainable head over pre-trained features: $\hat{D}_n =  F_n \circ C_n$. 

\noindent
Then, a model selection mechanism is proposed to select the pre-trained models whose of-the-shelf feature spaces best distinguish samples from real and fake distributions. Specifically, the union of the real images $\{ x_i \}$, and generated images $\{ G(z_i) \}$ is split into the training and the validation set. Then, for each pre-trained model, the classification head is trained on the training set and validated on the validation set. The model with higher validation accuracy is considered a better one to be ensembled with $D$ during training GAN.
In practice, they first train the GAN with a conventional adversarial loss (or simply use a well-trained GAN as initialization), and then after a certain amount of epochs, they progressively add $\hat{D}_n$ and use an ensemble of discriminators. Empirical results show that in general, GAN can benefit from up to three additional off-the-shelf models ($N=3$).
They also use data augmentation \cite{karras2020ada, zhao2020diffaug} and label smoothing \cite{salimans2016improved}, and interestingly, the experimental results suggest that under limited data the ensemble learning of GAN can not converge without using the data augmentation.
Experimental results also show that using the pre-trained vision models as only discriminator is not helpful for training GAN, and only ensemble learning can improve the performance. 
Even though the ensembling of pre-trained vision models is very effective in training GANs under limited data, it adds a considerable amount of computational overhead, and the model selection scheme is shown to be noisy with a sample size of $\sim$100.



% GenCo - AAAI22
\subsection{Generative Co-training (Gen-Co)} 
Generative Co-training (Gen-Co) \cite{cui2022genco} uses multiple discriminators during training GAN under limited data to extract diverse and complementary information from available samples and prevent overfitting to these samples.
This co-training has to major modules: Weight-Discrepancy Co-training (WeCo) and Data-Discrepancy Co-training (DaCo). WeCo trains two separate discriminators $D_1$ and $D_2$, where both discriminators use the standard adversarial loss of the discriminator in GAN, and $D_2$ have an additional weight-sharing regularizer.
DaCo uses $D_1$ and $D_3$, where $D_1$ is the same as the one used in WeCo, but $D_3$ is using the frequency components of the real and fake images (extracted by a random frequency component rejection based on the Fourier transform \cite{huang2021fsdr, huang2021rda}) to perform the real-fake classification task.
The idea of using multiple discriminators in GenCo \cite{cui2022genco} is similar to DAG \cite{tran2021dag}, and it prevents overfitting by capturing and ensembling different and complementary information from limited data. Experimental results show that using GenCo with data augmentation approaches like DiffAugment \cite{zhao2020diffaug} can provide further improvement.



% When, Why, and Which Pretrained GANs Are Useful?  - ICLR22
\subsection{Revisit Transfer Learning in GANs} \citet{grigoryev2022when} revisit the transfer learning from a pre-trained GAN to different target domains with the na\"ive fine-tuning approach similar to TGAN \cite{wang2018tgan} but using StyleGAN2-ADA \citet{karras2020analyzing, karras2020ada} structure as a modern GAN structure, instead of WGAN-GP \cite{gulrajani2017improved} used in TGAN.
Results in \citet{grigoryev2022when} suggest that for recent GANs, it is beneficial to transfer the knowledge from sparse and diverse sources rather than dense and less diverse ones, \ie, for most of the target distributions, using the pre-trained StyleGAN2 on ImageNet is an excellent start point despite the fact that StyleGAN2 trained on ImageNet have poor visual quality (FID $\approx$ 49.8).

\noindent
The contribution of the pre-trained $G$ and $D$ in generating images from the target domain under transfer learning is analyzed using a synthetic experiment. The results suggest that the pre-trained $G$ is responsible for covering the modes of target data (by guaranteeing diverse sample generation in initialization), and pre-trained $D$ is responsible for the initial gradient field to guide the generated samples to proper data regions.
The quality of pre-trained $G$ is evaluated by recall measure \cite{kynkaanniemi2019improved}, and the quality of the pre-trained $D$ is measured by the similarity between the gradient field of the generated samples and the vector field of the 'golden` ground truth gradients \cite{sinha2020top} that points towards the closest mode.
Further analysis in \cite{grigoryev2022when} shows that transfer learning from a pre-trained GAN covers more models from the target distribution and decreases the training time due to more gradual image evolution during training compared to training from scratch.
Apart from the interesting analysis performed in \cite{grigoryev2022when}, the major limitation is that it considers the StyleGAN-2 as representative of all SOTA GAN structures.




% StyleGAN-NADA - ACM Transaction on Graphics'22
\subsection{StyleGAN-NADA} \citet{gal2022stylegannada} address the problem of {\em zero-shot} image generation by adapting a pre-trained GAN to the target domain without seeing any images from the target domain and using just text prompts (\eg, Photo$\rightarrow $Sketch). 
Specifically, StyleGAN-NADA \cite{gal2022stylegannada} uses CLIP \cite{radford2021CLIP} to guide the adaptation of the pre-trained GAN into the target domain using text prompt as input.
CLIP is a foundational model for joint vision-language representation. It is trained on image-text pairs with a contrastive learning goal and maps both image and text into a powerful multimodal embedding space. StyleGAN-NADA aims to answer the following two key questions: (1) What is the best way of distilling the semantic knowledge encapsulated in CLIP space? (2) How CLIP-based optimization should be regularized to prevent mode collapse or adversarial solutions? 

One of the pioneers for using CLIP-based guidance in generative models is StyleCLIP \cite{patashnik2021styleclip} where the following loss is used for editing image attributes:
\begin{equation}
    \mathcal{L}_{\texttt{StyleCLIP}} = D_{\texttt{CLIP}}(G(z),t_{target})
\end{equation}
where $t_{target}$ is textual description, and $D_{\texttt{CLIP}}$ is the cosine distance in CLIP space.
This loss is designed for CLIP-guided image editing and when applied to the zero-shot problem, it leads to adversarial solutions or mode collapse as it sees no benefits in maintaining the diversity of the pre-trained GAN.
To overcome this issue, a directional CLIP loss is proposed where it tries to identify the CLIP-space direction between source and target domains and fine-tune the $G$ in a way that generated images differ from the source domain only along this direction.
As there is no image from the target domain, the textual prompts for source and target domains are used to determine the direction of embedding change as follows:
\begin{equation}
\label{eqn:text_direction_stylegannada}
    \Delta T = E_T(t_{traget}) - E_T(t_{source})
\end{equation}
 After finding this direction, the pre-trained generator is duplicated. One of the generators is kept frozen $G_{frozen}$. Another one --named $G_{train}$-- is trained in a way that for the same latent code, the generated image differs from the $G_{frozen}$'s only along the direction determined by the textual prompt.
Specifically, the direction of change on the generated images using two generators can be determined as:
\begin{equation}
\label{eqn:image_direction_stylegannada}
    \Delta I = E_I(G_{train}(z)) - E_I(G_{frozen}(z))
\end{equation}
where $E_I$ denotes CLIP's image encoder.
Then, the directional loss is designed to align these two direction changes:
\begin{equation}
    \mathcal{L}_{direction}=1-\frac{\Delta T.\Delta I}{|\Delta T||\Delta I|}
\end{equation}
Note that during adaptation, the latent space mapping layer of StyleGAN ($z \rightarrow \omega$) is kept frozen, and only Conv layers are updated. However, following previous works in FSIG, they constrain the updates into a limited set of parameters.
Specifically, in each iteration of training, StyleGAN-NADA selects only $k$ layers to update and the remaining layers are kept frozen during that iteration. These $k$ layers are identified by measuring the most changed latent mapping functions using $\mathcal{L}_{\texttt{StyleCLIP}}$.
In addition, they have used a latent mapper mechanism (similar to StyleCLIP) to shit the latent codes to the region of the target class and prevent the adapted generator from generating images from both source and target domains.




% MindTheGAP - ICLR'22
\subsection{MindTheGap}
\citet{zhu2022mindthegap} apply a similar idea to StyleGNA-NADA to tackle the one-shot image generation problem.
In principle, StyleGAN-NADA can solve this problem by replacing the text direction in Eqn.\ref{eqn:text_direction_stylegannada} with the direction attained by the available sample from the target domain $I_{B}$ as follows:
\begin{equation}
    \Delta I^{'} = E_I(I_{B}) - \frac{1}{|A|} \sum_{I_A \in A} E_I(I_A)
\end{equation}
where $\frac{1}{|A|} \sum_{I_A \in A} E_I(I_A)$ denotes the mean embedding of the images in domain A (source).
However, using mean embedding leads to diversity loss. In fact, one major challenge in this setup is to find a more specific and accurate match for a given $I_B$, to get a meaningful direction on CLIP space. 
The key idea of the MindTheGap \cite{zhu2022mindthegap} is to address this problem by replacing the mean embedding with the embedding of the projection of $I_B$ into the source domain. More specifically, the Improved-Image2StyleGAN (II2S) GAN inversion technique \cite{zhu2020improved} is used to find the extended latent code $\omega^{ref}$ for target image $I_B$ in the GAN pre-trained on the source domain. Then, this source code is used to generate the projection of the $I_B$ in the source domain: $I^*_A = G_A(\omega^{ref})$. 
Then, the source to target direction in CLIP space is computed as follows:
\begin{equation}
    \Delta I^{''} = E_I(I_{B}) - E_I(I_{A}^*)
\end{equation}
Then, similar to StyleGAN-NADA, GAN adaptation is done by aligning the direction of change in pre-trained GAN and adapted GAN (Eqn.\ref{eqn:image_direction_stylegannada}) with $ \Delta I^{''}$ through a directional loss:
\begin{equation}
    \mathcal{L}_{direction}^{'}=1-\frac{\Delta I^{''}.\Delta I}{|\Delta I^{''}||\Delta I|}
\end{equation}
In addition, to make sure that the direction proposed by using $I_B$ and the corresponding projected image in source domain $I_A^*$ is accurate, a reconstruction loss is added to this directional loss. This reconstruction loss has two components: (1) a similarity loss between the CLIP embeddings of $I_B$ and the inverted image in the target domain $G_B(\omega^{ref})$, (2) reconstruction loss between $I_B$ and $G_B(\omega^{ref})$ using perceptual (measured by LPIPS) and pixel-level (measured by MSE in image space) accuracy.
In addition to using the cross-domain direction for updating GAN, an additional regularizer is used that makes sure the changes within the domain are the same for both source and target domains. More specifically, for a specific extended latent code $\omega$, the within domain change in target domain is computed as $\nu_B = E_I(G_B(\omega)) - E_I(I_B))$. Similarly, the within domain change in the source domain is computed as $\nu_A = E_I(G_A(\omega)) - E_I(I_A^*))$. Then, a regularizer is used to align these changes.
Finally, after training GAN using the combination of these losses, \citet{zhu2022mindthegap} have observed that in some cases, even though the content is changed properly, the style is still similar to the style of the source domain. To mitigate this issue, they partition the extended latent space of the adapted GAN into two parts: $\omega = [\omega_c, \omega_s]$. Here $\omega_c$ encodes content and consists of the first $m=7$ blocks of extended latent space.  
Similarly, $\omega_s$ encodes the style and consists of the remaining blocks of extended latent space. 
They keep the $\omega_c$ same and modify $\omega_s$ by making it the weighted combination of the styles of current GAN and the style code in inverted $I_B$: $\hat{\omega}_s = (1-\alpha)\omega_s + \alpha \omega_s^{ref}$, where $\omega_s^{ref}$ is last $(18-m)$ blocks of $\omega^{ref}$.


% One CLIP - arXiv'23
\subsection{One-Shot Adaptation of GAN in Just One CLIP}
One-Shot Adaptation of GAN in Just One CLIP (OneCLIP) \cite{kwon2022oneclip} exploits the CLIP embedding to handle GAN inversion, cross-domain consistency, and patch-level consistency for one-shot image generation.
More specifically, first, similar to MindTheGAP \cite{zhu2022mindthegap} a reference latent code is computed for a target image using the GAN inversion technique. However, to improve the accuracy of the inversion, in addition to spatial loss and perceptual loss, the difference between the inverted sample and target sample in the CLIP embedding space is also added to the optimization objective.
Results show that using CLIP embedding can considerably improve the inversion performance.
OneCLIP also uses a cross-domain consistency similar to CDC \cite{ojha2021cdc} to preserve the diversity of the source $G$ during adaptation. However, instead of using the features extracted by $G_s$ and $G_t$, the CLIP embeddings of generated images before and after adapting $G$ are used to compute the cross-domain loss.
In addition, to preserve the local consistency, a patch-wise contrastive learning approach is applied. For this, some random patch locations are selected, and the patches in these locations are cropped from both images generated by $G_s(z_i)$ and $G_t(z_i)$. Two patches from $G_s(z_i)$ and $G_t(z_i)$ in the same location are considered positive pairs and others are considered negative pairs.
Contrastive learning is applied in the CLIP embeddings of the patches.



\noindent
{\color{magenta} \bf Remark.} Path-level processing; contrastive learning; GAN inversion.


%Check TargetCLIP for HyperDomainNet

%%% HyperDomainNet - NeurIPS'22
% Assuming that enough details about StyleGAN-NADA and MindTheGAP are given before
%\noindent
\subsection{HyperDomainNet} 
HyperDomainNet \cite{alanov2022hyperdomainnet} proposes three main contributions for zero/one-shot image generation using StyleGAN2 \cite{karras2020analyzing} guided by the feedback from CLIP \cite{radford2021CLIP}. First, they propose a modulation scheme that decreases the trainable parameter space when adapting a pre-trained StyleGAN2 to a target domain.
More specifically, during adaptation, all parameters of the source GAN $G_s$ are frozen and only these domain modulation (DomMod) parameters are being trained to adapt the model to the target domain.
Note that in StyleGAN2 \cite{karras2020analyzing}, within each style block, the convolution weights $w$ are first modulated by incoming style as follows:
\begin{equation}
    \label{eqn:style_modulation}
    w^{'}_{ijk} = s_i . w_{ijk}
\end{equation}
where $w^{'}$ denotes modulated weights, $s_i$ is the corresponding scale to the $i^{th}$ input feature map, and $j$ and $k$ enumerate the output feature map and spatial footprint of the convolution, respectively.
Then, the modulated weights are normalized using the demodulation operation:
\begin{equation}
    \label{eqn:style_demodulation}
    w^{''}_{ijk} = \frac{w^{'}_{ijk}}{\sqrt{{\sum_{i,k} w^{'}_{ijk}}^2 + \epsilon}}
\end{equation}
where $\epsilon$ is a small positive value used to prevent numerical issues. This modulation/demodulation has been replaced with standard adaptive instance normalization (AdaIN) \cite{ulyanov2016AdaIN} used in StyleGAN \cite{karras2019style} to perform normalization based on the expected statistics of input feature maps rather than forcing them explicitly. Then, the {\em domain-modulation} proposed in \cite{alanov2022hyperdomainnet}, is applied as an additional modulation in each style block of StyleGAN2, after standard modulation in Eqn.\ref{eqn:style_modulation} as follows:
\begin{equation}
    \label{eqn:domain_modulation}
    \hat{w}^{'}_{ijk} = d_i . w^{'}_{ijk}
\end{equation}
Then, domain-modulated weights $\hat{w}^{'}_{ijk}$ are normalized using Eqn.\ref{eqn:style_demodulation}. The main idea behind this domain modulation is to freeze source GAN parameters and optimize domain parameters $\{d_i\}$ when adapting a GAN to a target domain.
This scheme is applied to $\mathcal{L}_{direction}$ of StyleGAN-NADA (Eqn.x), and MindTheGap (Eqn.xx) for zero-shot and one-shot image generation using the feedback from CLIP feature space. However, the optimization is performed \wrt domain modulation parameters instead of whole parameters in the synthesis network. This reduces parameter space by 4000X (updating 6K parameters in \cite{alanov2022hyperdomainnet} instead of 24M parameters in \cite{gal2022stylegannada, zhu2022mindthegap}) with comparable expressiveness power when adapting to close domains.
Second, \cite{alanov2022hyperdomainnet} proposes a regularizer to improve the diversity using the feedback from CLIP space in one-shot domain adaptation \cite{zhu2022mindthegap}. For this, for the batch of generated images by source and target GANs, the similarities/differences in the CLIP feature space between each pair are preserved using the following loss term:
\begin{equation}
    \mathcal{L}_{\texttt{indomain-angle}} = \sum_{\substack{i,j=1 \\ i \neq j}}^n \{<E_I(G^s(z_i)), E_I(G^s(z_j))> - <E_I(G^t(z_i)), E_I(G^t(z_j))> \}^2
\end{equation}
where $E_I$ denotes CLIP's image encoder. Finally, they propose HyperDomainNet $D_{\varphi}$ which is learned to generate the domain parameters given the input target domain, \eg for the zero-shot generation it uses embeddings of the text obtained by CLIP's text encoder to generate modulation parameters $d_{\mathcal{D}_i}=D_{\varphi}(E_T(t_{\mathcal{D}_i}))$. This structure enables multi-domain zero/one-shot image generation and is used in two different setups: learning to generate parameters for seen domains or generating modulation parameters for unseen domains.


% IPL - CVPR'23
\subsection{Zero-shot Image Generation with Image-specific Prompt Learning (IPL)}
\citet{guo2023ipl} mention that one issue with StyleGAN-NADA \cite{gal2022stylegannada} is that the direction of the update from a source domain to a specific target domain is fixed for all images which leads to an identical supervision signal.
To improve this, an image-specific prompt learning (IPL) approach is proposed which aims to learn a specific text prompt for each image in the source GAN, and then apply the learned prompt for zero-shot image generation from a target domain.
Specifically, for a latent code $\omega^i$, the generated image by the source generator is denoted as $G_s(\omega^i)$, and a latent mapper is proposed to learn to generate the image-specific prompt matrix for this latent code as follows:
\begin{equation}
    F(\omega^i,\theta) = [V]_1^i [V]_2^i ... [V]_m^i
\end{equation}
where $[V]_j^i$ is the $j^{th}$ embedding representing a prompt vector.
Then, the domain embedding $[Y_s]$ is added to this prompt to represent both the prompt and the domain:
\begin{equation}
    M_s^i =F(\omega^i,\theta)[Y_s] = [V]_1^i [V]_2^i ... [V]_m^i [Y_s]
\end{equation}
To train the mapper function $F$, given a batch of latent codes $\{ \omega^1, \omega^2, ..., \omega^n \}$, a batch of corresponding prompt matrices can be generated as $\{ M_s^1, M_s^2, ..., M_s^n \}$ by $F$, and a batch of corresponding images $\{ G_s(\omega^1), G_s(\omega^2), ..., G_s(\omega^n) \}$ can be generated by $G_s$.
Then the $n \times n$ pairs $<G_s(\omega^i), M_s^j>$, $i,j \in \{1,2,...,n\}$ have been used in a contrastive manner to train $F$, where pairs on $i=j$ are taken as positive pairs, and pairs on $i \neq j$ are taken as negative pair. Contrastive learning is performed in the CLIP space, where CLIP's image encoder and text encoder are used to encode the generated images and text prompts, respectively.
An additional domain regularization loss is used to prevent learning the negative prompts for the target domain.
After training mapper $F$, it is plugged into a directional loss similar to StyleGAN-NADA \cite{gal2022stylegannada} to adapt the GAN for image generation from the target domain.




% CLIP-Sculptor - CVPR'23
\subsection{CLIP-Sculptor: Zero-Shot Generation of Shapes}
\citet{sanghi2023clipsculptor} proposes CLIP-Sculptor to use the CLIP guidance for zero-shot shape generation.
CLIP-Sculptor is trained in three steps.
In the first step, a vector quantized variational auto-encoder is trained to reconstruct a voxel input.
Two different resolutions of VAEs are trained ($32^3$, and $64^3$) for computational efficiency.
Then, in the second step, a coarse transformer is designed that takes $4^3$ masked codes and the embedding of the training images (encoded by CLIP image encoder) to generate the conditional $4^3$ latent codes.
Finally, in the third step, a fine transformer is trained which takes the output latent code $4^3$ from the previous step, and a high-resolution masked $8^3$ latent code to generate the high-resolution latent code $8^3$.
Then, during inference, the text encoder of the CLIP embeds the input text into CLIP space. This embedding is fed into the trained coarse transformer to generate low-resolution latent code which is fed to the fine transformer for outputting the high-resolution latent code.
Finally, the generated latent code is fed into the voxel decoder to output the desired shape.

\noindent
{\color{magenta} \bf Remark.}
There are some other few-shot shape detection works that can be briefly mentioned here.

\subsection{CF-Font: Content Fusion for Few-shot Font Generation}
{\color{red} ---updating---}

% DnaGAN - SIGGRAph-Asia'22
\subsection{Dynamic Few-shot adaption of GAN (DynaGAN)} 
Dynamic Few-shot adaption of GAN (DynaGAN) \cite{kim2022dynagan} uses a similar idea to HyperDomainNet \cite{alanov2022hyperdomainnet} where it adapts a pre-trained GAN to multiple domains using the same adaptation scheme of the MindTheGap \cite{zhu2022mindthegap} but by only updating some modulation parameters. Specifically, DynaGAN modulates the normalized weights within the synthesis block of StyleGAN2 (same as HyperDomainNet) and also adds a residual weight to the input weights (before the modulation operator in the synthesis block). Since DynaGAN adds a residual weight for every single parameter in the convolutional layer, to prevent parameter explosion, these residual weights are generated by rank-1 tensor decomposition \cite{hou2021parameter} through the outer product of multiple learnable vectors \cite{milad2021revisit, simon2020modulating}.
Additionally, to enable automatic image generation for multiple domains, a mapping network is trained to generate the modulation network for a target domain conditioned on some input (in the form of image embedding) from that domain. 

%% FreGAN- NeurIPS'22
% Assuming that enough details about FastGAN are given before
%\noindent
\subsection{Frequency-Aware GAN (FreGAN)} 
Building on top of FastGAN\cite{liu2021fastgan}, FreGAN \cite{yang2022fregan} aims to improve the image generation of GANs in limited data regimes by increasing frequency awareness of $G$ and $D$. GANs are notorious for their spectral bias \cite{rahaman2019nnfrequncybias, khayatkhoei2022ganfrequencybias}, \ie preferentially fitting to low-frequency components and tending to ignore high-frequency components in data distribution \cite{durall2020watchupconvolution, tancik2020fourier, chandrasegaran2021closer, dzanic2020fourier}. As high-frequency components encode finer details of an image \cite{gonzales1987digital}, missing them can harm the image generation performance. FreGAN \cite{yang2022fregan} shows that this problem worsens under limited data, where the details of generated images deteriorate (\eg mixing scene details in a generated landscape painting), even using approaches like FastGAN \cite{liu2021fastgan} which highly curates network structure for limited data setup. FreGAN applies the Haar wavelet transform \cite{porwik2004haar} using low ($L$) pass filter $L^T = \frac{1}{\sqrt{2}}\big[1,1\big]$, and high ($H$) pass filter $H^T = \frac{1}{\sqrt{2}}\big[-1,1\big]$, which in each iteration gives one sub-image with low-frequency component $LL$, and three sub-images with high-frequency components $LH$, $HL$, and $HH$ containing details in vertical, horizontal, and diagonal directions, respectively. Then, three modules are proposed utilizing these frequency components to increase GAN's frequency awareness.
First, the high-frequency discriminator is considered to give high-frequency feedback to $D$ when distinguishing real and fake images. More specifically, denoting $HF_D^i = LH_D^i + HL_D^i + HH_D^i$ as high-frequency information attained by applying wavelet transform on features of $i^{th}$ layer of $D$, these features are used to construct the high-frequency adversarial loss as follows: 
\begin{equation}
    \mathcal{L}^{HF} = 
    \mathbb{E}_{x \sim p(x)} \{ min(0,-1+D(HF_D[x]))\} + 
    \mathbb{E}_{z \sim p(z)} \{ min(0,-1-D(HF_D[G(z)]))\}
\end{equation}
By optimizing this adversarial loss ($\arg \min_G \max_D \mathcal{L}^{HF}$), $D$ uses high-frequency information to distinguish real and fake images, and $G$ tries to generate samples with similar high-frequency distribution to real data to deceive $D$. Second, they propose Frequency Skip Connection to prevent the loss of high-frequency information of $G$. For the $i^{th}$ feature map of $G$, the frequency spectrum is extracted using wavelet transform, resulting in $LL_G^i, LH_G^i, HL_G^i, HH_G^i$ sub-images. Then, this frequency information is added to the feature maps of the next layer:
\begin{equation}
    F^{'}_{i+1} = F_{i+1} + Unpooling(LL_G^i, LH_G^i, HL_G^i, HH_G^i)
\end{equation}
where $Unpooling$ denotes wavelet unpooling operation \cite{yang2022fregan}. Finally, as $G$ has no access to the frequency information of the real data during training, an additional constraint is considered by aligning the frequency components of a generated image extracted from $G$ and $D$. More specifically, the high-frequency information of the $G$'s $i^{th}$ feature map for an input $z$ is computing by discarding $LL_G^i$, and summing all others: $HF_G^i(z) = LH_D^i + HL_D^i + HH_D^i$. Similarly, the high-frequency information of the $D$'s $i^{th}$ feature map is denoted by $HF_D^i(z)$. Then, for each feature map, an additional regularizer is considered during GAN training to penalize the difference between high-frequency information extracted by $G$ and $D$: $\mathcal{L}_{align} = \parallel HF_D^i - HF_D^i\parallel_{1}$.


% DigGAN - NeurIPS'22
% assuming that local attractors information from FastGAn is discussed before
%\noindent
\subsection{Discriminator gradIent Gap regularization for GAN (DigGAN)} 
In \cite{fang2022diggan}, it has been shown that during training a GAN with limited data, the Discriminator gradIent Gap (DIG) between real and generated images is increasing. More specifically, \cite{fang2022diggan} defines DIG as the gap between i) the norm of the gradient of $D$'s prediction \wrt real images, and ii) the norm of the gradient of $D$'s prediction \wrt generated images, as follows:
\begin{equation}
\label{eqn:dig}
    R(D,x_R, x_F) = \Big(\Big\| 
   \frac{\partial D}{\partial x_R} \Big\|_2 - \Big\| 
   \frac{\partial D}{\partial x_F} \Big\|_2 \Big)^2
\end{equation}
where $x_R$, and $x_F$ denote real and generated images, respectively. Experimental results show that when training a BigGAN \cite{brock2019biggan} on $10\%$ of CIFAR-100 \cite{krizhevsky2009cifar100}, the DIG defined in Eqn. \ref{eqn:dig} is increasing during training as opposed to a nearly stable value during training of the same BigGAN on the whole CIFAR-100 dataset. 
Note that the gradient in Eqn. \ref{eqn:dig} can be interpreted as the $D$'s output changes when the input image changes and the norm of this gradient show the magnitude of this rate. Therefore, a large DIG value can be considered as an imbalance between $D$'s rate of change \wrt real and generated images. Therefore, $D$ learns faster on either real or generated images resulting in training instability.
Based on this observation, \cite{fang2022diggan} hypothesizes that increasing DIG during training GAN under limited data results in unstable training of GAN and thereby performance degradation (higher FID values). To mitigate this issue, DigGAN adds the DIG term as a regularizer to $D$'s loss during training (leaving $G$'s loss unchanged):
\begin{equation}
    \mathcal{L}_D = \mathbb{E}_{x \sim p(x)} \{-D(x)\} +  \mathbb{E}_{z \sim p(z)} \{D(G(z))\} + 
    \lambda \mathbb{E}_{x \sim p(x)} \mathbb{E}_{z \sim p(z)} 
    \Big(\Big\| 
   \frac{\partial D}{\partial x} \Big\|_2 - \Big\| 
   \frac{\partial D}{\partial G(z)} \Big\|_2 \Big)^2
\end{equation}
To reduce the variance of change during training, the moving average of the norm term is used. An analysis is also proposed for the simple task of generating two real values in \cite{fang2022diggan} to show the effectiveness of DigGAN against local attractors \cite{liu2021fastgan}. Specifically, this analysis shows that while vanilla GAN may stuck in a local attractor and can not escape it, DigGAN can evade these attractors, and even escape them if training starts from a local attractor. \textcolor{cyan}{\em An explanation about the local attractor should be added after reviewing the FastGAN paper.} Experimental results show that the proposed regularizer is orthogonal to the data augmentation approaches \cite{zhao2020diffaug}, and combining these two can provide a further performance improvement.

% DynamicD- NeurIPS'22
\subsection{Dynamin Capacity for Discriminator (DynamicD)} 
\citet{yang2022dynamicd} focuses on importance of $D$ for training GANs from the perspective of task hardness \cite{tran2019taskhardness} handled by $D$. Considering the bi-classification task handled by $D$, as the quality of the generated data by $G$ evolves during training, this bi-classification task appears to be {\em time-varying}, in contrast to common image classification tasks where training data remains unchanged. So, DynamicD \cite{yang2022dynamicd} proposes that one solution to handle this time-varying task more efficiently is to use a $D$ with {\em dynamic capacity} during training.
The importance of aligning the model capacity with task hardness is considered in existing studies on image classification \cite{zhang2017understanding, he2016identity, he2016resnet}, where either under-fitting can happen when using a model with less capacity than what is required, or over-fitting can happen due to over-parametrization (unnecessarily high capacity). 
As an example, for the ImageNet classification \cite{deng2009imagenet}, ResNet-50 \cite{he2016resnet} has worse performance than ResNet-101 as it is not capable enough to handle complex distribution. For the same task,  ResNet-200 has a worse performance compared to ResNet-152 due to over-parametrization. 

\noindent
The dynamic capacity is proposed for two different scenarios based on the quantity of available data for GAN training. In the first scenario, when sufficient data is available, the intuition is that the bi-classification task becomes more challenging as the training proceeds ---generating noisy images with $G$ in early iterations and more realistic ones in later ones. Therefore, DynamicD increases the capacity of $D$ as training goes on. More specifically they change the capacity of a standard convolutional layer by varying the dimension of the input and output channels as follows:
\begin{align*}
    c_{out} \times c_{in} \times k \times k \rightarrow  (1+\alpha)c_{out} \times (1+\alpha)c_{in} \times k \times k
\end{align*}
where $c_{in}$ and $c_{out}$ denote the number of input and output channels, $K$ is spatial size of convolutional kernel, and $\alpha$ is extending coefficient. For applying DynamicD on training GAN with sufficient data, they vary $\alpha$ from -0.5 to 0 during training and use StyleGAN2 as baseline GAN. Therefore, training starts with a half-baseline $D$ and ends with baseline $D$. The architecture of $G$ is kept the same as the baseline.

\noindent
In the second scenario, training GAN with limited data is considered where usually over-fitting occurs in later stages of training \cite{yang2022dynamicd}. Therefore, in this case, DynamicD uses a decreasing capacity scheme using a shrinking coefficient $\beta$. Concretely, during a certain training iteration and for a given $\beta$, a sub-kernel with the form of $\beta c_{out} \times \beta c_{in} \times k \times k$ is randomly sampled from each convolutional layer of $D$. During training $\beta$ is varied from 1 to 0.5 using StyleGAN2 as the baseline, resulting in a half-baseline $D$ when training is completed.
Conceptually, this strategy not only decreases network capacity but also to some extent introduces multiple $D$s using random sampling. The analysis in \cite{yang2022dynamicd} suggests that these multiple discriminators can complement each other and therefore mitigate overfitting under limited data. 
Note that as DynamicD has overall less capacity than the baseline for $D$, and it introduces no additional parameters or loss function, the computational complexity of this approach is less than baseline GANs and performs better in the same setup. In addition, for limited data setup, it can be combined with both data augmentation approaches \cite{karras2020ada} and transfer learning-based approaches \cite{mo2020freezed} to give further improvements.
However, the major limitation of DynamicD is that the design of making $D$ dynamic is done manually (moving from half-baseline to baseline or vice versa). Considering the number of available samples from the target domain, using a self-adjusting strategy for determining capacity in each training iteration, or using AutoML ideas like neural architecture search \cite{wang2021alphanet} can improve the performance. 

%%% MaskedGAN - NeurIPS'22
\subsection{Masking Images for GAN training (MaskedGAN)} 
\citet{huang2022maskedgan} randomly masks out certain image information during training GAN with limited data, to {\em improve $D$'s understanding} on real images.
Specifically, \cite{huang2022maskedgan} hypothesizes that under limited data, $D$ tends to minimize the loss on the real/fake classification task by resorting to less meaningful shortcuts of either memorizing the training data or merely attending to easy-to-discriminate image locations and spectra. Therefore, $D$ achieves a poor understanding of real data and its feedback is not useful enough for $G$ to generate realistic images. 
A similar problem of learning trivial solutions has been previously observed in unsupervised/self-supervised learning, where masked auto-encoders (MAEs) are applied to tackle this problem. 
In MAEs, {\em image masking} is the core design to evade trivial solutions and learn high-level semantic features \cite{bao2022beit, he2022maskedautoencoder, vincent2010stacked, vincent2008extracting}. As an example, \cite{he2022maskedautoencoder} shows that using a high-ratio masking strategy in MAEs can impede learning shortcuts (\eg recover a masked patch by interpolating adjacent image patches) in image reconstruction, and encourage the model to learn nontrivial and meaningful representations (\eg recover a masked patch by modeling a global inter-patch relationship). 

Inspired by the recent success of MAEs in self-supervised learning \cite{he2022maskedautoencoder}, MaskedGAN \cite{huang2022maskedgan} utilizes a similar idea for training GANs under limited data by masking both spatial and spectral domains.
%They propose that due to spectral bias in GANs, in addition to the spatial domain, this masking should also be applied to the spectral domain. 
First, they perform an analysis to confirm that under limited data, $D$ resorts to meaningless shortcuts. Specifically, they have shown that Gini Coefficient \cite{dorfman1979ginicoeff} of discriminator's spatial attention increases quickly during training.
The Gini coefficient has a reverse relation with equality \cite{dorfman1979ginicoeff}, \ie, the large Gini coefficient of $D$ in the image generation task, shows that the discriminator focuses more on some spatial locations (probably easy to discriminate) and ignores other spatial locations (hard to discriminate), leading to an over-confident $D$ which gives poor feedback to $G$ for image generation.


% Hi Touba
% Let me put a draft that captures the whole points of the paper. Later we can edit this and make it shorter when we are moving to ver 1.0 of the survey. bashe! Mokhlesam!

For spatial masking, they first generate a random patch-based mask. The grid size of the mask is $N \times N$, which results in patch size $\frac{H}{N} \times \frac{W}{N}$ for an image with the spatial size $H \times W$. Then a random spatial shift $\xi \in [0:\frac{H}{2N}, 0:\frac{W}{N}]$ is applied to the generated mask resulting in a shifted random mask: $\mathbb{M}_{spatial} = x \odot m_{spatial}$. Note that using this shift, the masked patch can appear in any location, instead of appearing only on the fixed grid usually used in MAEs \cite{bao2022beit, he2022maskedautoencoder}, as image generation requires high-fidelity along the spatial location.

For spectral masking, first, the Fourier transform (FT) is used to extract the frequency representation of the image. Following \cite{huang2021rda, zhang2022spectral} they used a decomposition after FT to obtain $C$ different frequency channels. 
The information within each channel can be obtained by summing the whole frequency content on that channel. 
Then, they normalized the frequency information of each channel by the sum of information in all channels and used the normalized information of each channel as the probability of masking that channel, \ie, channels with more information are being masked more frequently. The spectral masking $\mathbb{M}_{spectral}$ is applied after the spatial one resulting in the following masking operation:
\begin{equation}
    \mathbb{M}(.) = \mathbb{M}_{spatial}(\mathbb{M}_{spectral}(.))
\end{equation}
Note that by applying this masking operation on the real images, task hardness is increased for $D$ which may result in an imbalance between the learning pace of $D$ and $G$ and impede proper learning of useful features. To prevent this, the same masking operation is also applied to the generated images to sparsify the training signal and slow down $G$'s training. Therefore, the training objective of MaskedGAN \cite{huang2022maskedgan} can be written as follows:
\begin{equation}
    \mathcal{L}_d = 
    \mathbb{E}_{x \sim p_{data}} \{f_d[-D(\mathbb(M(x))] +
    \mathbb{E}_{z \sim p_{z}} \{f_d[D(\mathbb(M(G(z)))]
\end{equation}
\begin{equation}
    \mathcal{L}_g = 
    \mathbb{E}_{z \sim p_{z}} \{f_g[-D(\mathbb(M(G(z)))]
\end{equation}
Note that as two masking strategies are designed in orthogonal spaces, they complement each other, and encourage $D$ to learn a more holistic understanding of real images and surpass trivial solutions.
MaskedGAN is also shown to be modeled as a Two Time-Scale Update Rule \cite{heusel2017twotimescale} which supports its convergence to a Local Nash Equilibrium under certain conditions. 
MaskedGAN is shown to be effective for both CNN-based architectures (conditional image generation with BigGAN \cite{brock2019biggan} on ImageNet, unconditional image generation with StyleGAN2 \cite{karras2020analyzing}) and transformer-based structures (unconditional image generation on TransGAN \cite{jiang2021transgan} and GANformer \cite{hudson2021ganformer}).

\noindent 
{\em Remark.}
As mentioned before, FastGAN \cite{liu2021fastgan} uses a similar intuition of evading attention on specific areas of real images, and designs an auto-encoding scheme to enforce $D$ to learn more comprehensive features. However, the difference is that while FastGAN uses shallow structures to prevent over-fitting, the MaskedGAN keeps the high capacity of $G$ and $D$, and manipulates the way that data is exposed to these networks, and in this way, it can enjoy representative power of deep models under limited data. 




\subsection{Generalized One-shot Image Generation} 
\citet{zhang2022generalizedoneshot} defines a new task on top of one-shot image generation which considers entity transfer: "Train a GAN to generate high-quality and diverse images from the target domain, given a pre-trained GAN, a reference target image $x_{ref}$ with some entity and related entity mask $m_{ref}$".
The adapted generator $G_t$ consists of two parts: I) $\hat{G}_t$ initialized with a pre-trained StyleGAN2 generator which is responsible for creating the images from the target domain (same style as $x_{ref}$ but borrowing content from the pre-trained GAN), II) an auxiliary network $g_{aux}$ which is being trained from scratch, and is responsible for generating entities (\eg mask, hat, eyeglasses, etc).

\noindent
Adapting $\hat{G}_t$ and training $g_{aux}$ has multiple steps.
First, the reference image $x_{ref}$ is mapped into the replicated latent space ($\omega$) of the pre-trained StyleGAN2 using GAN inversion technique in \cite{tov2021designing} to obtain related latent code $\omega_{ref}$.
Then, GAN is trained by reconstruction loss $\mathcal{L}_{rec}$ ---which includes negative structural similarity \cite{wang2004image}, perceptual loss \cite{zhang2018unreasonable}, and mean squared errors--- to reconstruct the target image $\hat{x}_{ref}$ using the same latent code $\omega_{ref}$.
Next, the latent code is made style-frozen. Specifically, assuming that in StyleGAN2 the earlier part of the latent code $ \omega_{ref}= [\omega_{ref}^{c}; \omega_{ref}^{s}]$ is responsible for the content ($\omega_{ref}^{c}$), and the later part is responsible for the style ($\omega_{ref}^{s}$),  the style part is kept the same for all generated images, and the content part can be varied to generate different images with that style.
Two additional regularizers are used during this final adaptation step. 
Inspired by the fact that the internal patch distribution of a single image contains reach information, the divergence of the internal distribution between the reconstructed image and each generated image is minimized by imposing a regularizer using slice Wasserstein distance \cite{bonneel2015sliced} on the extracted features of two images.
In addition, to preserve the cross-domain correspondence and prevent collapsing to a single mode, the variant Laplacian regularizer ---applied on CLIP\cite{radford2021CLIP} features of generated images with source and adapted generator--- is added to the final loss term. 
One particular limitation of this work is that there is no metric to assess the successful transmission of the entity to that target domain instead of subjective evaluation, where other methods lack any mechanism to transfer these entities. Other evaluation metrics are also based on face detection/recognition networks that may suffer from domain shift when used in these distant domains (\eg Disney face).

\subsection{Introducing editable and representative attributes for few-shot image generation (DFSGAN)}
\citet{yang2023dfsgan} proposed two major contributions for training GANs with limited data.
First, instead of sampling the latent code from a Gaussian distribution, a GMM with M components is used to model the latent code to improve the diversity of the generated samples. Second, the content and layout information in the intermediate layers of the $G$ is preserved by extracting channel-wise information and spatial information on these layers using additional modules and scaling the intermediate features of the $G$ based on these extracted features.


\subsection{Re-GAN: Data-Efficient GANs Training via Architectural Reconfiguration}
\citet{yang2022fregan} proposes a series of consecutive pruning and growing steps to find a sparse GAN and full-version counterpart that improves the GAN's performance and computation/data efficiency under both large-scale and limited data scenarios.


\noindent
\textcolor{violet}{\bf
Episodic-Learning Based Approaches
} 

\noindent
\textcolor{magenta}{\bf Remark.} For this section we may include a generic framework that discusses the learning form task in episodic learning (FSC), and then discuss how this is applied to the few-shot image generation.


%\noindent
%\textcolor{magenta}{{\bf Remark.} \textcircled{\raisebox{-0.9pt} {1}} LoFGAN has good writing about the problem setup, some evaluation details, and categorization of different approaches that can be useful when discussing the general setup for this part.
%\textcircled{\raisebox{-0.9pt} {2}} One limitation regarding this line of work about their strong assumption on the image space is also nicely mentioned in this work: `other works consider that auxiliary dataset and limited dataset are form different image domain but in this work we consider that these two datasets are from the same image domain but are disjoint in the label space'. This can be included when we are discussing the differences between two lines of works.
%}

\subsection{Data Augmentation Generative Adversarial Networks (DAGAN)}
DAGAN \cite{antoniou2017dagan} leverage the task of the learning augmentation manifold to the standard learning process of the GAN. The augmentation manifold is modeled as some transformations on the input, and then, the generator is conditioned on this transformation to generate images.
After training the generator, these transformations are considered to be general and can be applied to the new sample from the unseen classes to generate diverse images based on the learned augmentation manifold. 


% GMN --- AISTATS2018
\subsection{Generative Matching Networks (GMN)}
GMN \cite{bartunov2018few} is one of the first works that uses meta-learning approaches to train a generative model for few-shot image generation, however, it is not using the GAN as the generative model. More specifically, it uses the idea of MatchingNet \cite{vinyals2016matching} to train a generative model using the variational approach for generating images from a new domain using a few available samples.


\subsection{Few-shot Image Generation with Reptile (FIGR)} 
\citet{clouatre2019figr} 
is the first work that uses the meta-learning approach to train a GAN for generating images from a few seen samples.
More specifically, it defines a setup for FSIG inspired by the counterpart problem setup in the few-shot image classification widely used in meta-learning approaches as the running example.
In this setup, the aim is to find a set of parameters $\theta$ that can converge to a random FSIG task with a few data from that task and the limited (no) training iterations.
In this setup, the FSIG task is defined for each class separately. For example, for class $i$, there are a set of FSIG tasks: $\mathcal{T}_i = \{ \mathcal{T}_i^j \}$, where $\mathcal{T}_i^j$ is a $1$-way $k$-shot image generation task, constructed by randomly sampling $k$ images form class $i$. 
The model is supposed to learn to generate diverse and high-quality samples from class $i$ where only $k$ real samples from that class are available.
To handle this challenging task, the model is trained using episodic learning which matches the condition in which the model is trained and tested. 
More specifically, \cite{clouatre2019figr} meta-trains a GAN model with $\theta = \{ \theta_g, \theta_d \}$, where $\theta_g$ and $\theta_d$ denote the parameters of the generator and discriminator, respectively. 
During training (meta-training), the set of training tasks $\{ \mathcal{T}_i \}_{i=1}^{N}$ are constructed using the training classes, where each $\mathcal{T}_i$ consists of hundreds of task generated by randomly sampling $k$ images from that task. The model is learned on the meta-training tasks and then evaluated on similar FSIG tasks from unseen classes. For example, for the MNIST dataset \cite{lecun1998gradient} which consists of handwritten digits, the meta-training tasks can be constructed using the digits $0,\dots,8$, \ie  $\{ \mathcal{T}_0, \dots, \mathcal{T}_8 \}$, and the evaluation (meta-test) tasks using the unseen class during training, \ie, $\mathcal{T}_9$.

\noindent
Meta-learning approaches usually consist of an inner loop and outer loop updating scheme, where the model adapts to training data at the inner loop, and the meta-parameters are updated at the outer loop. FIGR uses the Reptile \cite{nichol2018reptile} meta-learning algorithm which is a first-order approximation of the well-known MAML approach \cite{finn2017maml}.
More specifically, during each training iteration, FIGR clones the current parameters $W_g=\theta_g$, $W_d=\theta_d$, and samples a task $\mathcal{T}_i^j$ from training tasks. Then, it uses $k$ samples of that task together with generated samples (by $W_g$) to get the loss and update both $W_g$ and $W_d$ in an adversarial manner, resulting in new parameters for GAN: $W_g^i$ and $W_d^i$.
Then, the difference between the updated parameters during the inner loop and the initial GAN parameters is used to update the GAN in the outer loop:
\begin{align*}
  & \theta_g \leftarrow \theta_g -  W_g^i
  \\
  & \theta_d \leftarrow \theta_d -  W_d^i
\end{align*}
During training, the $\theta = \{ \theta_g, \theta_d\}$ is expected to learn the knowledge across all training FSIG tasks, and be able to adapt to an unseen FSIG task $\mathcal{T}_i$ (FSIG tasks from class $i$ are not represented to the model during training) by observing only $k$ samples and applying only the adversarial training of the inner loop. Note that in this setup, a labeled dataset is required to generate the tasks separately.

\subsection{Domain Adaptive Few-Shot Generation framework (Dawson)} 
Domain Adaptive Few-Shot Generation framework (Dawson) \cite{liang2020dawson} claims that the main limitation of applying optimization-based meta-learning approaches like MAML \cite{finn2017maml} and Reptile \cite{nichol2018reptile} in the problem setup of the \cite{clouatre2019figr} is that the loss of the generator in the inner loop of meta-learning is not calculated \wrt training data but provided by the discriminator.
To address this problem, \cite{liang2020dawson} modifies the inner loop training. Specifically, it adopts the discriminator to training data of the meta-training task to return the loss that is supposed to come from the training data, and the discriminator is updated by the evaluation dataset to provide the loss supposed to be calculated on the evaluation set.


\subsection{Fast Adaptive Meta-Learning (FAML)}

Similar to FIGR \cite{clouatre2019figr}, Fast Adaptive Meta-Learning (FAML) \cite{phaphuangwittayakul2021faml} uses Reptile \cite{nichol2018reptile} to update the weights of the generative model for few-shot image generation.
However, instead of using the standard GAN structure, it uses an encoder-decoder architecture for the generator and adds the reconstruction loss to the main objective.

\subsection{Contrastive Meta-Learning
Generative Adversarial Network (CML-GAN)}
CML-GAN \cite{phaphuangwittayakul2022cmlgan} uses a similar approach to FAML \cite{phaphuangwittayakul2021faml} but with leveraging contrastive learning to learn quality representations.

\subsection{Matching-based Few-shot Image Generation (MatchingGAN)}  \citet{hong2020matchinggan} proposes a matching generator and discriminator to learn to generate images from unseen categories using limited data from that category. The matching generator consists of three encoders and one decoder and the matching discriminator consists of a single network as the discriminator.
The whole system can be seen as a fusion model that uses two of the encoders to extract the similarity between the embedding of random noise and the training (conditioning) images. This similarity is then used as the interpolation coefficient by a UNet-shaped \cite{ronneberger2015unet} auto-encoder that extracts the embeddings of the training images and fuses them for constructing the new image.
The matching generator and matching discriminator are trained using the adversarial training of GAN.
In addition, a reconstruction loss in the spatial domain, and a feature matching loss using the feature maps extracted by the discriminator are used in the generator loss to stabilize the training procedure and make sure the generated sample is similar to the training images.
MatchingGAN also uses the class conditional loss \cite{odena2017conditional} for the discriminator as an additional supervisory signal. 
Once trained, at test time no fine-tuning is required, and the generator of the MatchingGAN fuses the images from an unseen category to generate new images from the same category.
Note that since the FSIG task is performed separately for each class at test time, different from the conditional GANs, there is no conditioning on the $G$ regarding the class label.


\noindent
In the problem (training) setup of the MatchingGAN (and most probably all follow-up works), it divides the available labeled data into training, validation, and test set.
Then for each class of the training data (where a minimum of 100 images for each class is available), it generates a 3-shot 1-way conditional image generation task (conditioning is not applied as an input to $G$ and is just used in the $D$, but the few-shot generation task just considers one class) and trains the model based on these training tasks.
At test time, for each class, a 3-way 1-shot task is created by sampling from the corresponding unseen class, and this is repeated 128 times to compute the FID for that category, meaning that for each class the network has access to $128 \times 3 = 384$ images.
This will probably get averaged over all unseen classes to report the FID (FID calculation for one class is mentioned in the paper but the details of the final FID value are not provided in the paper).
The point is that we can train a FastGAN \cite{liu2021fastgan} (ProtoGAN \cite{yang2023protogan}) completely from scratch using these 384 images and probably get better results.
However, one strength of such approach is that they have shown that usign MatchingGAN as an augmentation can drastically improve the performance of the few-shot image classification.

\noindent
Another limitation of this setup is that for each k-shot 1-way generation task, one image is generated. If additional images are generated, what would be the diversity as this method heavily relies on the conditioned images?
The labeled data is also required to train these models!

\noindent \textcolor{cyan}{This work could be explained in a bit more detail (a figure for the network structure and including some equations) as it's the pioneer one and the others can be summarized.}


\subsection{Fusing and Filling GAN (F2GAN)} 
Fusing and Filling GAN (F2GAN) \cite{hong2020f2gan} uses a similar idea to the MatchingGAN to fuse the given few-shot images from the same category and generate a new image. However, instead of finding the similarity between random noise and few-shot images (done in MatchingGAN), F2GAN uses random coefficients to fuse the given images and obtain the low-level (general) information, and then the details of the fused image is extracted using an attention mechanism. The generator in F2GAN has a UNet-shaped structure, where the corresponding layers of the encoder and decoder are connected with a non-local attention fusion module.
The attention module takes the weighted average (scaled by the same random coefficients) of the real image features from the encoder and the corresponding features from the decoder as input and produces the image details by attending to local regions of the real images encoded by the encoder.
Similar to MatchingGAN, the discriminator is trained by a combination of an adversarial loss and a class conditional loss.
An image reconstruction loss and a mode-seeking loss are also added to improve training stability and increase image generation diversity.
One interesting observation in the \cite{hong2020f2gan} is that $k=3$ is the optimal shot for this setup and adding more images brings slight improvement compared to the additional complexity introduced. Similar behavior is also reported previously for meta-learning-based few-shot image classification approaches \textcolor{cyan}{[to find and include the citation]}.

\subsection{Local Fusion GAN (LoFGAN)} \citet{gu2021lofgan} mentions that there are two major limitations with previous fusion-based approaches that use the image-level (global) weighted average as fusion strategy \cite{hong2020matchinggan, hong2020f2gan}: i) when input images are not semantically aligned, fused feature map would also be misaligned which may result in aliasing artifact in the output image, ii) as the relative positions of each local semantic are fixed during image-level fusion, this reduces the generation diversity.
Local Fusion GAN (LoFGAN) \cite{gu2021lofgan} aims to address these limitations using a local fusion to focus on local features (pixel positions) instead of global features (image-level).
Specifically, similar to the previous works, LofGAN uses a UNet-shaped generator (including an encoder and a decoder) and a discriminator. 
Given $k$ input images, the LofGAN uses one of them as the base image and the remaining $k-1$ images as the reference set which acts like a feature-bank for that base image to generate the new image.
It introduces a local fusion module between the encoder and decoder which consists of three steps. 
First, after extracting the features of all images, a local selection step simply samples $n$ pixel positions from $h \times w$ as the ones that should be replaced for generating the new image.
Then the similarity between each selected position in the base image and all of the positions in each reference image is calculated and the most similar pixel content from each reference image is determined and used in a weighted average to generate the fused feature map.
The fused feature map is then passed as input to the decoder to generate the new image.
In addition to standard adversarial loss, a class-conditional loss is also used during training.
Finally, to stabilize the training process, a reconstruction loss is used similar to \cite{hong2020matchinggan, hong2020f2gan}. However, in order to prevent the aliasing effect, in contrast to \cite{hong2020matchinggan, hong2020f2gan} that uses image-level reconstruction loss, \cite{gu2021lofgan} uses the local construction loss that creates a reconstructed local image based on the indices learned in local fusion model.
Note that similar to previous fusion-based methods, this method also struggles with the one-shot scenario.



\subsection{Adaptive multi-scale modulation GAN (AMMGAN)}
Adaptive multi-scale modulation GAN (AMMGAN) \cite{li2023ammgan} aims to utilize the multi-scale semantic information to improve the image generation performance.
It uses a UNet-shaped generator where instead of the skip connection, an adaptive fusion mechanism is used for learning pixel-wise metric coefficients for the fusion process.
The reconstruction loss is also tailored \wrt the semantic metric used for fusion. 


\subsection{WaveGAN} 
\citet{yang2022wavegan} uses the same structure as LofGAN \cite{gu2021lofgan} as the baseline and proposes additional modules to improve the frequency awareness and therefore the image generation performance. 
Similar to \cite{gu2021lofgan}, the generator consists of an encoder and a decoder.
The Haar wavelet transform \cite{porwik2004haar} is applied on the feature maps $F^i$ of the encoder to extract the frequency components: $LL^i$, $LH^i$, $HL^i$, and $HH^i$. 
Then, a skip connection is introduced in the encoder that feeds the low-frequency information ($LL^i$) of the previous layers to the next layers to ensure proper encoding of this information and increase the fidelity of the generated images.
For the decoder, the high-frequency information of the $F^i$ (\{$LH^i$, $HL^i$, $HH^i$\}) is first inverted to the feature space using an inverse transformation and then added to the respective layer of the decoder to improve the amount of detail in the reconstructed image. For the inverse transform, inspired by LoFGAN's feature selection, an index-based selection mechanism is proposed which is shown to be more effective than using the mean inverse transform.
Additionally, a frequency-based reconstruction loss is proposed that aims to regularize the frequency difference between the generated and real images to make sure that generated images are not biased towards a specific frequency spectrum.



\subsection{DeltaGAN}
\citet{hong2022deltagan} aims to increase the image generation quality by learning the difference between real images (delta), and then using this delta concept in generation. 
DeltaGAN includes a reconstruction subnetwork and a generation subnetwork.
The reconstruction subnetwork takes a pair of real images as input and uses one as the base image and the other as the target image.
Then, using a series of encoders, it estimates a delta between these two real images $\Delta_r$ that is sufficient to reconstruct the target image from the base image. 
More specifically, a generator $G$ takes the encoded feature map of the base image $E_c(x_b)$ and the real delta $\Delta_r$ to reconstruct the target image.
In the generation subnetwork, the fake delta $\Delta_r$ between a random noise $z$ and the same base image is estimated, and then used for the sample generation.
The encoder and the generator used in the generation subnetwork are the same as the ones used in the reconstruction subnetwork which allows the knowledge transfer between these two subnetworks.
These subnetworks are trained using adversarial loss, class-conditional loss, and reconstruction loss similar to previous works.
An additional adversarial delta training is proposed which aims to close the gap between the real and fake deltas, where the discriminator tries to distinguish the real and fake deltas, while the generator aims to deceive the discriminator.

\noindent
\textcolor{magenta}{\bf Remark.} There is an interesting experiment in this paper that compares DeltaGAN with CDC in the Supp. and shows that both have similar performance in the flower dataset, but CDC requires adaptation.
However, the comparison is not fair as they have used just one image for fine-tuning the CDC as opposed to 128 tasks in DeltaGAN which probably uses 128 images in test time.
A fair investigation could be interesting!



%It consists of a reconstruction network and a generation network. The reconstruction network learns the delta between real images and how to apply this delta to reconstruct a target image by learning some encoders and a decoder (generator).
%The encoders and decoder are shared with the generation network that aims to generate diverse images using input noise and a reference image.
%These two networks are trained in an adversarial manner with concatenating a set of discriminators.
%DeltaGAN follows the MatchingGAN setup. It also uses a classifier for seen classes during training making it a conditional GAN. But note that the difference with standard conditional GAN is that it is supposed to generate images from unseen categories. But again it sees a few data from that categories but not being learned for that particular label.


\subsection{Few-shot Image Generation Using Discrete Content Representation (Disco)}

FUNIT \cite{liu2019funit} is a popular image-to-image translation approach that disentangles the content and style and fuses the content of the source images with the style of the target image for image translation.
Disco \cite{hong2022disco} uses a similar approach with a VQ-VAE-like framework for few-shot image generation.
More specifically, it learns a dictionary based on the seen images to encode input images to visual tokens.
These tokens are then fed into the decoder with the style embedding of the seen images to generate images from unseen classes.




\subsection{Attribute Group Editing (AGE)}
Attribute Group Editing (AGE) \cite{ding2022age} captures the useful transformation as some category-irrelevant attributes that can be learned using seen categories and then transferred to the unseen categories for diverse image generation.
The category-irrelevant attributes are learned in $\mathcal{W}^+$ space of a StyleGAN2 \cite{karras2020analyzing}.
More specifically, the GAN inversion is used to invert the samples of a category to $\mathcal{W}^+$ space, and the mean latent code for all samples of a category is used as the embedding of that category and all differences are considered as category-irrelevant attributes.
These attributes are modeled using sparse dictionary learning as an encoder-decoder structure.
After learning the sparse dictionary, it is used to generate the attributes for the unseen images combined with random noise.
This attribute is added to the inverted latent code of the unseen image and then fed to the pre-trained StyleGAN2 on the seen classes to generate new samples from the unseen class.
Stabel AGE (SAGE) \cite{ding2023sage} extends AGE by addressing the class inconsistency by taking all given samples from unseen classes into account during inference.




\subsection{Hyperbolic Attribute Editing (HAE)}
Hyperbolic Attribute Editing (HAE) \cite{li2022hae} uses a similar idea to AGE \cite{ding2022age} for capturing the attributes in the latent space and then transferring these attributes to the unseen classes.
However, instead of using Euclidian distance, the learning, and editing are performed in the Hyperbolic space which allows more control on the semantic diversity.
Latent codes are projected from Euclidian space to Hyperbolic space using a hyperbolic feedforward layer \cite{chami2019hyperbolic}.



%------------------------------------------
\clearpage
\noindent
\textcolor{magenta}{\bf Man's edit from here.}

\subsection{DreamBooth}
\citet{ruiz2023dreambooth}
proposes a new task of  {\em Subject-Driven Generation} (SDG). Although SDG's setup is similar to few-shot image generation (FSIG), there are important differences. For SDG, given a few images of {\em the same subject}, the goal is to generate a diverse set of images of {\em the same subject} in novel contexts with natural interactions 
between the subject and new
contexts. SDG focuses on both maintaining high fidelity to the key visual features
of the subject and generating images in diverse and novel contexts.
On the contrary, 
for FSIG, we are given a few images of {\em the same target domain}, but in most cases, the subjects in the images are different, e.g., human faces of different identities. With the pre-trained generative model (for TL approach), the goal is to generate a diverse set of images of {\em the same target domain}.




In \cite{ruiz2023dreambooth}, they propose to achieve SDG by fine-tuning 
a pre-trained text-to-image model, e.g. Imagen \cite{saharia2022photorealistic}, DALL-E2 \cite{ramesh2022hierarchical}, in order to  implant  
into the model 
the subject instance paired with a text prompt containing a unique identifier and the name of
the class the subject belongs to (e.g., ``A [V] dog'').
They further propose a class-specific prior preservation loss to encourage diversity and to mitigate {\em language drift}, i.e., the model progressively loses syntactic and semantic knowledge during fine-tuning.











% FSIG   

% SDG 

% A few images of the same subject are given.

% The goal is to generate a diverse set of images with the same subject under novel contexts.



% Fair generative modeling

% A few images of the same source domain under fair distribution w.r.t. some sensitive attributes  are given.

% The goal is to generate a diverse set of images of the same source domain with fair distribution.


 

\begin{table}[h]
\centering
\begin{tabularx}{\textwidth}{|X|X|X|}
\hline
Task 
& Limited samples given in the task 
& Goal of the task \\
\hline
Few-shot image generation
(FSIG) \cite{ojha2021cdc,zhao2022adam}
& A few images of {\em same target domain} are given. Often,  the subjects in the images are different although they belong to the same domain.
& The goal is to generate a diverse set of images of the {\em same target domain}.  \\
\hline
Subject-driven generation (SDG) \cite{ruiz2023dreambooth} 
& A few images of the {\em same subject} are given.
& The goal is to generate a diverse set of images with the {\em same subject under novel contexts}. \\
\hline
Fair generative modeling \cite{teo2023fairtl}
& A few images of the {\em same source domain under fair distribution} w.r.t. some sensitive attributes  are given. 
& The goal is to generate a diverse set of images of the {\em same source domain with fair distribution}. \\
\hline
\end{tabularx}
\caption{Comparison of several tasks based on fine-tuning a pre-trained source generative model using limited samples.}
\end{table}


\subsection{DISP}

Focusing on GANs,
\citet{mangla2021disp}
proposes a transfer learning method DISP. 
Particularly, they leverage
informative image prior from a pre-trained network on a rich source domain for image generation.
For extracting image prior, they use the last layer activations of Vgg16 \cite{simonyan2014very}
classification network trained on ImageNet 
and that of  SimCLR \cite{chen2020simclr}
 trained using self-supervised learning on ImageNet.
DISP shows competitive performance in a range of setups from limited training samples to large-scale:
(1) 25 - 100 images, (2) 2k - 5k images, (3) 50k- 1M images.



\subsection{LSO} 

\citet{zheng2023lso} proposes
a latent space optimization  
for conditional StyleGAN.
They project the few-shot samples into the latent space of the conditional StyleGAN in order to localize the latent subspace of an unseen category defined by a category vector.
They propose 
adversarial loss and semantic stabilization loss in order to refine the latent subspace of the unseen category.
Using 3 datasets (Flowers \cite{nilsback2008automated}, AnimalFaces \cite{liu2019fewshot}, VGGFaces \cite{cao2018vggface2}), they demonstrate injecting unseen classes into the conditional StyleGAN using 1 or 3 images of the unseen classes.


\subsection{FakeCLR}

In
\citet{li2022fakeclr}, the authors  
analyze 3 different contrastive learning strategies, namely Instance-real,  Instance-fake and 
Instance-perturbation. They find that Instance-perturbation
contributes the most improvement in quality. They show that Instance-perturbation can effectively alleviate the issue of latent space discontinuity. They further propose techniques to improve upon Instance-perturbation.
They demonstrate competitive performance in the range of 100 to 5K training samples based on StyleGAN2 architecture.


\subsection{KD-DLGAN}

In \citet{cui2023kddlgan}, the authors propose KD-DLGAN,  a knowledge distillation 
 (KD) approach for training GAN under limited data. 
KD 
\cite{hinton-distill,chandrasegaran2022revisiting}
in machine learning refers to a technique where a large, complex model (known as the teacher model) is used to train a smaller, more compact model (known as the student model). The goal of KD is to transfer the knowledge and insights learned by the teacher model to the student model.
KD is effective in overcoming  model overfitting and  improving generalization performance.
In
\cite{cui2023kddlgan}, 
they 
 leverage pretrained vision-language model CLIP \cite{radford2021CLIP} as the teacher model  to 
distill text-image knowledge  to the discriminator, in order to mitigate 
 discriminator overfitting.
Instead of using vanilla KD, they propose two designs that are suitable for image generation tasks:  aggregated generative knowledge distillation (AGKD) and correlated generative knowledge distillation (CGKD).
AGKD mitigates the discriminator overfitting with harder learning tasks and distills general knowledge from the
pretrained model. 
CGKD  improves the generation diversity by distilling and preserving the diverse
image-text correlation from the pretrained model.
They demonstrate effectiveness of their approach in unconditional generation using 
StyleGAN2 with 100 to 389 samples, and 
conditional generation using BigGAN with 
sampling of 
CIFAR-10/CIFAR-100 (5K, 10K, 50K) and 
ImageNet (25K, 50K, 100K).


\subsection{SCHA-VAE}

In \citet{pmlr-v162-giannone22a}, 
the authors  extend  latent variable models for sets
to a fully hierarchical approach, and propose 
SCHA-VAE for Set-Context-Hierarchical-Aggregation Variational Autoencoder for few-shot generation. 
They  explore
likelihood-based model comparison, iterative data
sampling, and adaptation-free out-of-distribution
generalization. 
They demonstrate their proposed SCHA-VAE outperforms baseline
Variational Autoencoder
(VAE) - which does not explore set information -  
and
Neural Statistician (NS) \cite{edwards2016towards}
in few shots (2 to 20) of 
Omniglot, MNIST and several other datasets.











 

 











%------------------------------------------
\clearpage
\noindent
\textcolor{blue}{\bf Chris Edits:}

\subsection{SINE: SINgle Image Editing with Text-to-Image Diffusion Models}

\textcolor{blue}{[Chris: Note that this work goal is very similar to Dreambooth 1) Retain subject 2) Alter context. Approach however is different with additionally contribution (flexible resolution). ]}

\citet{zhang2023sine} introduces SINE which aims to improve on single-image editing by fine-tuning a pre-trainied diffusion model based on a single image, while leveraging on classifier free guidance to alter the context. Additionally, SINE enables flexible resolutions output \ie there is no fixed resolution output, through the use of patch based fine-tuning. Specifically, 
SINE achieves this in two stages, fine-tuning then editing. 
In fine-tuning,
SINE 
takes two inputs consisting of patches from the target image, and a text-prompt consisting of a unique identifier followed by a class (\eg "A photo of a [*] class").
Then with these inputs, it
fine-tunes only the denonising module  $\epsilon_\theta$ and the text-encoder module $\tau_\theta$ of a pre-trained Latent Diffusion Model (LDM) \cite{rombach2022latentdiffusion}.
%It does this by taking in inputs consisting of patches from the target image, and a text-promot consisting of a unique identifier followed by a class (\eg "A photo of a [*] class").
We denote the modified denonising and text-encoder modules by $\hat{\epsilon}_\theta$ and $\hat{\tau}_\theta$, respectively.
During editing, for the first $T-K$ steps, SINE then linearly combines the scores from both the modified modules ($\hat{\epsilon}_\theta$,$\hat{\tau}_\theta$) and the pre-trained models (${\epsilon}_\theta$,${\tau}_\theta$), where both set of modules take the same noise input $\mathbf{z}_t$, but while $\hat{\tau}_\theta$ takes the same text-prompt in the fine-tuning stage, $\tau_\theta$ instead takes a new target text-prompt intended for editing the image. The remaining $K$ steps are then denoised by $\hat{\tau}_\theta$ only. 

\subsection{SinDiffusion}
\citet{wang2022sindiffusion} introduces SinDiffusion that aims to improve upon weakness in SinGAN \cite{shaham2019singan} when learning the internal patch distribution of a single image.
Specifically, it aims to address artifacts observed in SinGAN, which the authors attribute to the propagation of small errors during progressive training. In contrast, SinDiffusion circumvents this problem by removing the need for progressive growing due to its use of a diffusion model architecture. Furthermore, the authors propose that in order to improve sample diversity, the size of the receptive field should be reduced. This is achieved by
%adjusting the size of the receptive field by 
reducing the depth of the denoising network, as well as the number of time-embedding Resblocks.
%to further improve sample diversity.
SinDiffusion demonstrates competitive performance for scene generation, with samples from the Place50 dataset (a subset of the Place356 \cite{zhou2017places} dataset).

\subsection{SinDDM: A Single Image Denoising Diffusion Model}
\citet{kulikov2022sinddm} proposes the use of a multi-scale diffusion process capable of 
learning the internal distribution of the single training image.
%tackling multiple task from a single image \eg style transfer, harmonization and externally supervised generation.
SinDDM involves the standard forward and backwards diffusion process but at progressive scales.
This allows the model to learn both coarse grain and fine grain details.
%Specifically, during the forward diffusion process, the source training image is first down-sampled. Then at each scale $s$, a combination of a blurred up-sampled version and the orignal down-sampled version are forward diffused.
Specifically, at each scale $s$ in the forward diffusion process, SinDDM learns to diffuse a combination of the down-sampled training image and a blurry variant. Then during backwards diffusion, the model learns to simultaneously denoise and deblur to output the generated image. 
They demonstrate the effectiveness of this approach for multiple tasks, unconditional image generation at different resolutions, text-guided generation, generation with guided region of interest, style transfer and image harmonization.

\subsection{DEff-GAN: Diverse Attribute Transfer for Few-Shot Image Synthesis}

\citet{kumar2023deffGAN} explore the problem of learning the internal distribution for $k$ images, thereby allowing for the potential mixing of different image semantics and hence improving diversity.
To tackle this challenge, they propose Deff-GAN, a multi-scale training pyramid approach consisting of multiple generators $G_i$ and discriminator $D_i$ for $i\in[0,N]$, where \{$G_0$,$D_0$\} and \{$G_N$,$D_N$\} learn the coarsest and finest details, respectively.
Specifically, at each scale, the $G_i$ are first trained completely. Then their layers are concatenated to the next training scale $G_{i+1}$. Through this implementation, Deff-GAN extends upon the single-image model setups, to be able to handle multiple images. Furthermore, under these multiple images \eg 2 samples Deff-GAN, demonstrates being able to generate more diverse images.


\subsection{BlendGAN: Learning and Blending the Internal Distributions of Single Images by Spatial Image-Identity Conditioning}

\citet{kligvasser2022blendgan} introduces BlendGAN, which explores learning the internal patch distribution from multiple images thereby allowing for new applications \ie morphing, melding and structural-texture fusion.
Specifically, BlendGAN conditions their training image on a one-hot spatial image identity, $img_{id}$ that is utilized for spatial adaptive normalization to modulate the generator's feature maps.
Furthermore, BlendGAN utilizes a multi-scale pyramid approach, where each scale contains a generator and discriminators pair, $\{G_{i},D_{i}\}$. %Then the generated samples from each $G_{i}$ are upsampled and appended 
Overall, BlendGAN demonstrates to be effective on both single and multiple image settings, where under the latter settings more application can be tackled \eg mixing of images.

%\textcolor{blue}{[To update]}
\subsection{SinFusion: training diffusion models on a single image or video}

\citet{nikankin2022sinfusion} introduces SinFusion which explores learning the internal patch distribution from both a single image or multiple images (video) to generate diverse new samples for dynamic scene extrapolation. 
SinDiffusion extends on DPPM \cite{ho2020denoising} and reduces the size of the receptive fields by first removing attention layers, then adopting ConvNext \cite{liu2022convnet} blocks in the U-Net \cite{ronneberger2015unet} architecture. 
Additionally, cropped images are input into the model (as opposed to multi-scale pyramid approaches).
To reconstruct videos, a series of images \ie $\{x_0^1,x_0^2,\dots,x_0^N\}$ are used as inputs  into a series of 3 identical models. The first model predicts the next frame conditioned on the previous frame; the second model denoises and removes small artefacts from the generated images; the last model interpolates between the different frames. Additionally, the authors found that while the first model utilizes the standard denoising loss function, the second and third model demonstrates better performance with a reconstruction loss: 
\begin{equation}
    \mathcal{L}(\theta)=\mathbb{E}_{\mathbf{x_0},\epsilon} [|\mathbf{x_0}-\tilde{x}_{0,\theta}(x_t,t)|_2]
\end{equation}
Here, $\mathbf{\tilde{x}_0}$ is the constructed sample and $\theta$ are trainable parameters of the diffusion model. 

\subsection{MultiDiffusion: Fusing Diffusion Paths for Controlled Image Generation}

\citet{bar2023multidiffusion} proposes MultiDiffusion, a framework for controllable image generation that involves fusing the images from the existing pre-trained diffusion model while requiring no further fine-tuning.
Specifically, MultiDiffusion considers a pre-trained diffusion model, $\phi$, which operates on the images space $\mathcal{I}$ condition on some text prompts, $y\in \mathcal{Y}$. Then considering a set of mapping $F(.)$, the Multi-diffusion process aims to minimize the loss:
\begin{equation}
    \mathcal{L}=\sum_{i=1}^n|| W_i \otimes [F_i(J)-\phi(\mathcal{I}^i_t|y_i)] ||^2
\end{equation}
Intuitively, this is seen as minimizing the least square distance between the target generated images $J$ and originally generated images.

\noindent
\textcolor{blue}{
{\bf Two-sentence summary:}\\
\citet{bar2023multidiffusion} proposes MultiDiffusion, a post-processing method condition on pre-trained diffusion models.
MultiDiffusion uses patch-wise least square differences to fuse the outputs from conditional diffusion models without any training.
}

%\textcolor{blue}{Chris: Updating \dots}

\subsection{Target-Aware Generative Augmentations for Single-Shot Adaptation}
SiSTA \cite{thopalli2023targetaware}
aims to improve the downstream task of adapting a classifier to a target domain by learning a generative model to generate samples for that target domain using only one image. 
For this, a pre-trained generator is \textcolor{blue}{first} adapted to the target domain by enforcing the \textcolor{blue}{intermediate latent} output of the source discriminator to be the same for the available image and its reconstructed version by the source generator. 
\textcolor{blue}{Next, to improve diversity, SiSTA perturbs the latent representation of the fine-tune generator the falls below a threshold, either by replacing them with zero or reverting them back to the pre-trained generator's weights.}
\textcolor{blue}{Finally}, this generator is used for sample augmentation and adapting the classifier to the target domain.



%proposes an augmentation approach deployed in a single-shot adaptation setting. The work proposes a two-step process they refer to as \textit{SiSTA-G} and \textit{SiSTA-S}. \textit{SiSTA-G} involves itself with first inverting the provided single training images to its style-space latent vector, $\mathbf{W}^+$, followed by fine-tuning the pre-trained StyleGAN2 to target domain with the following loss function:
%\begin{equation}
  %  \mathcal{L}=arg \min_\theta \sum 
%\end{equation}
%\textcolor{blue}{Chris: Updating \dots}


\noindent
\textcolor{teal}{------------------------------------}

\noindent
\textcolor{teal}{[Milad]: Adding very recent works here}

\subsection{Rethinking Cross-domain Semantic Relation (CSR)}

Rethinking Cross-domain Semantic Relation (CSR) \cite{gou2023csr} uses a similar idea to CDC but applies the semantic loss directly to the spatial space, \ie, the generated images with $G_s$ and $G_t$.

\subsection{Progressive Few-shot Adaptation with Align-Free Spatial Correlation (ProSC)}
ProSC \cite{moon2023prosc} extends RRSA by performing a progressive adaptation to the target domain in $N$ iterations instead of a single adaptation.
The idea is that, in iterative adaptation, the domain gap between source $G_{n-1}$ and adapted model $G_n$ is less and more meaningful matches can be found to apply spatial alignment restrictions \citet{xiao2022rssa}.

\subsection{AutoInfoGAN}
AutoInfoGAN \cite{shi2023autoinfogan} builds on top of FastGAN \cite{liu2021fastgan} and applies a reinforcement learning-based neural architecture search to find the best network architecture for the generator.

\subsection{AdaptiveIMLE}
AdaptiveIMLE \cite{aghabozorgi2023adaptiveimle} adapts implicit maximum likelihood estimation \cite{li2018imle} to improve the mode coverage in generative learning under limited data. An adaptive version of IMLE is introduced which is more general with assigning different boundary radius for each sample. 

\subsection{Dynamically Masked Discriminator (DMD)}
Dynamically Masked Discriminator (DMD) \cite{zhang2023dmd} detects that the discriminator slows down learning and applies random masking to its features in an adaptive manner to balance its learning pace with the generator for GM-DC.



\clearpage


\noindent
{\textcolor{purple}{\bf ============ Keshik (Editing) =========}

\subsection{FS-MD: Few-shot Image Generation via Masked Discrimination}
Zhu \etal~\cite{zhu2022few} propose an approach for few-shot image generation using masked discrimination.
In particular, random masks are applied to features extracted by the discriminator (for both real and fake images) preventing the discriminator overfitting on the training samples. 
\cite{zhu2022few} posit that while masked discrimination can improve the diversity of adapted GANs, such approaches can weaken global image discrimination capabilities, resulting in lower quality of generated images.
To circumvent such quality degrade, cross-domain consistency (CDC) loss is applied to the discriminator to preserve the information learnt from the source domain (CDC loss is applied to the generator as well).
Although not discussed in the main paper in detail, this work applies both patch-level and image-level masked discrimination for calculating CDC loss.
They mainly conduct transfer learning experiments for 10-shot. Additional results on 5-shot and 1-shot are in Supplementary.
This paper deals with transfer learning under proximal domains (i.e.: FFHQ $\rightarrow$ Babies). 
They have 4 qualitative experiments on transfer learning under distant target domain (similar to CDC, DCL): FFHQ $\rightarrow$ Haunted Houses, LSUN-Church $\rightarrow$ Amedeo’s paintings, LSUN-Horse $\rightarrow$ Haunted Houses, 
LSUN-Horse $\rightarrow$ Amedeo’s paintings (Figure 25).
Even under domains of close proximity, we observe instances of incompatible knowledge transfer (i.e: transferring beard, moustache to Babies from FFHQ , Figure 18). 


\subsection{WeditGAN: Few-shot Image Generation via Latent Space Relocation}
WeditGAN \cite{duan2023weditgan} propose a fine-tuning based method for few-shot image generation (10-shot).
In particular, this work learns a constant offset parameter for the target domain ($\Delta w$) to relocate the source latent codes to target domain. i.e.:  $w_{src}~\rightarrow~w_{tgt}$. 
They also propose 2 improvements for WeditGAN: 1) Imposing perpendicular regularization on $\Delta w$ to facilitate accurate relocation, 2) fine-tuning the editing intensity for improving quality and 3) combining WeditGAN with contrastive loss.
In this work, the generator is frozen (both mapping and synthesis network in StyleGAN2) and the Discriminator is fine-tuned. 
This work deals with target domains with close proximity to the source domain.


\subsection{F3: Faster Few-Shot Face Image Generation with Features of Specific Group Using Pivotal Tuning Inversion and PCA}
F3 \cite{yuichi2023_fewshot} proposes a faster method to generate face images with features of a specific group. This is achieved by 2 steps: 1) PTI: GAN Inversion of target images followed by Pivotal tuning, 2) PCA: Used as a feature extraction strategy to render features of a specific group (i.e.: Japanese pop idols).
This work uses 100-shot data and StyleGAN-ADA architecture.

\subsection{DDPM-PA: Few-shot Image Generation with Diffusion Models}
\cite{zhu2022few_dm} introduces diffusion models (DM) for FSIG. 
Similar to GAN-based approaches, DMs overift under few-shot data (i.e.: 10-shot).
To alleviate overfitting, a transfer learning based approach is proposed.
The idea is to adapt pre-trained DMs to target domains with few-shot data. 
The authors argue that directly fine-tuning approach fails to retain diverse features and high frequency details (from the source domain).
Therefore, a pairwise adaptation method is proposed (DDPM-PA) which retains the relative distances between generated images during adaptation.
They also propose an additional method for high-frequency details enhancement. 
Overall, this work shows that transfer learning for DMs can be used for FSIG.



\subsection{AFI: Adaptive Feature Interpolation for Low-Shot Image Generation}
Dai \etal~\cite{dai2021implicit} propose an adaptive feature interpolation technique for generative modeling under limited data (i.e.: 100-shot).
This paper observes a flattening effect in discriminators with multiple output neurons, and takes advantage of this observation to propose an implicit data augmentation method in the feature-space of the discriminator. 
The results show that it can improve existing GAN baselines under limited data.


\subsection{DWSC: Dynamic Weighted Semantic correspondence for Few-Shot Image Generative Adaptation}
Hou \etal~ \cite{hou_dynamic} proposes 2 techniques to improve FSIG: 1) A dynamic weighted semantic correspondence between the source and target generator is introduced for better diversity (Pre-trained VGG19 features are used for perpetual loss).
2) To alleviate discriminator overfitting, a coupled training paradigm across the source and target domain to retain the feature extraction capabilities of the discriminator is proposed.



{\color{purple} Keshik: Beyond Image Generation}

\textbf{FS-3D-Shape: Few-shot 3D Shape Generation.} 
Zhu \etal~\cite{zhu2023fewshot_3d} study 3D shape generation under few-shot target data (10-shot shapes).
Given pre-trained 3D generative models on large source data, they adapt such models to target domain.
In particular, the optimization aims to retain the probability distributions of pairwise adapted samples both at feature-level and shape-level. 


\textbf{FS-SIS-CAT: Few-shot Semantic Image Synthesis via Class Affinity Transfer.}
Careil \etal~\cite{careil2023few} study the problem of few-shot semantic image synthesis which aims to generate photo-realistic images given semantic segmentation maps.
A transfer learning based approach called Class Affinity Transfer (CAT) is proposed.
This work uses both GANs and DMs for few-shot semantic image synthesis, and obtains photo-realistic results under 100-shot settings.


\textbf{CF-Font: Content Fusion for Few-shot Font Generation.}
Wang \etal~\cite{wang2023cffont} study font-generation which aims to transfer the source domain style to the target domain under a few-shot setting. In particular, a content fusion module and a projected character loss to improve the quality of skeleton transfer is proposed for few-shot font generation.


\noindent
{\color{purple} ========= End of Keshik (Editing) =========}

}



